Search for resonance-enhanced $CP$ and angular asymmetries in the $\Lambda^+_{c}\to p\mu^+\mu^-$ decay at LHCb

The first measurement of the $CP$ asymmetry of the decay rate ($A_{CP}$) and the $CP$ average ($\Sigma A_{\text{FB}}$) and $CP$ asymmetry ($\Delta A_{\text{FB}}$) of the forward-backward asymmetry in the muon system of $\mathit{\Lambda}^+_c\to p\mu^+\mu^-$ decays is reported. The measurement is performed using a data sample of proton-proton collisions, recorded by the LHCb experiment from 2016 to 2018 at a center-of-mass energy of 13$\text{ TeV}$, which corresponds to an integrated luminosity of 5.4$\text{ fb}^{-1}$. The asymmetries are measured in two regions of dimuon mass near the $\phi$-meson mass peak. The dimuon-mass integrated results are \begin{align*} A_{CP} &= (-1.1 \pm 4.0 \pm 0.5)\%,\\ \Sigma A_{\text{FB}} &= (\phantom{-}3.9 \pm 4.0 \pm 0.6)\%,\\ \Delta A_{\text{FB}} &= (\phantom{-}3.1 \pm 4.0 \pm 0.4)\%, \end{align*} where the first uncertainty is statistical and the second systematic. The results are consistent with the conservation of $CP$ symmetry and the Standard Model expectations.

==> Authorship_LHCb-PAPER-2024-051-arXiv.tex <==
LHCb collaboration:
R. Aaij,
A.S.W. Abdelmotteleb,
C. Abellan Beteta,
F. Abudin{\'e}n,
T. Ackernley,
A. A.  Adefisoye,
B. Adeva,
M. Adinolfi,
P. Adlarson,
C. Agapopoulou,
C.A. Aidala,
Z. Ajaltouni,
S. Akar,
K. Akiba,
P. Albicocco,
J. Albrecht,
F. Alessio,
M. Alexander,
Z. Aliouche,
P. Alvarez Cartelle,
R. Amalric,
S. Amato,
J.L. Amey,
Y. Amhis,
L. An,
L. Anderlini,
M. Andersson,
A. Andreianov,
P. Andreola,
M. Andreotti,
D. Andreou,
A. Anelli,
D. Ao,
F. Archilli,
M. Argenton,
S. Arguedas Cuendis,
A. Artamonov,
M. Artuso,
E. Aslanides,
R. Ata\'{i}de Da Silva,
M. Atzeni,
B. Audurier,
D. Bacher,
I. Bachiller Perea,
S. Bachmann,
M. Bachmayer,
J.J. Back,
P. Baladron Rodriguez,
V. Balagura,
A.  Balboni,
W. Baldini,
L. Balzani,
H.  Bao,
J. Baptista de Souza Leite,
C. Barbero Pretel,
M. Barbetti,
I. R. Barbosa,
R.J. Barlow,
M. Barnyakov,
S. Barsuk,
W. Barter,
J. Bartz,
J.M. Basels,
S. Bashir,
G. Bassi,
B. Batsukh,
P. B.  Battista,
A. Bay,
A. Beck,
M. Becker,
F. Bedeschi,
I.B. Bediaga,
N. A.  Behling,
S. Belin,
K. Belous,
I. Belov,
I. Belyaev,
G. Benane,
G. Bencivenni,
E. Ben-Haim,
A. Berezhnoy,
R. Bernet,
S. Bernet Andres,
A. Bertolin,
C. Betancourt,
F. Betti,
J.  Bex,
Ia. Bezshyiko,
J. Bhom,
M.S. Bieker,
N.V. Biesuz,
P. Billoir,
A. Biolchini,
M. Birch,
F.C.R. Bishop,
A. Bitadze,
A. Bizzeti,
T. Blake,
F. Blanc,
J.E. Blank,
S. Blusk,
V. Bocharnikov,
J.A. Boelhauve,
O. Boente Garcia,
T. Boettcher,
A.  Bohare,
A. Boldyrev,
C.S. Bolognani,
R. Bolzonella,
R. B.  Bonacci,
N. Bondar,
A. Bordelius,
F. Borgato,
S. Borghi,
M. Borsato,
J.T. Borsuk,
E.  Bottalico,
S.A. Bouchiba,
M.  Bovill,
T.J.V. Bowcock,
A. Boyer,
C. Bozzi,
J. D. Brandenburg,
A. Brea Rodriguez,
N. Breer,
J. Brodzicka,
A. Brossa Gonzalo,
J. Brown,
D. Brundu,
E. Buchanan,
L. Buonincontri,
M.  Burgos Marcos,
A.T. Burke,
C. Burr,
J.S. Butter,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
A. Caillet,
R. Calabrese,
S. Calderon Ramirez,
L. Calefice,
S. Cali,
M. Calvi,
M. Calvo Gomez,
P. Camargo Magalhaes,
J. I. Cambon Bouzas,
P. Campana,
D.H. Campora Perez,
A.F. Campoverde Quezada,
S. Capelli,
L. Capriotti,
R. Caravaca-Mora,
A. Carbone,
L. Carcedo Salgado,
R. Cardinale,
A. Cardini,
P. Carniti,
L. Carus,
A. Casais Vidal,
R. Caspary,
G. Casse,
M. Cattaneo,
G. Cavallero,
V. Cavallini,
S. Celani,
S.  Cesare,
A.J. Chadwick,
I. Chahrour,
H.  Chang,
M. Charles,
Ph. Charpentier,
E.  Chatzianagnostou,
M. Chefdeville,
C. Chen,
S. Chen,
Z. Chen,
A. Chernov,
S. Chernyshenko,
X.  Chiotopoulos,
V. Chobanova,
M. Chrzaszcz,
A. Chubykin,
V. Chulikov,
P. Ciambrone,
X. Cid Vidal,
G. Ciezarek,
P. Cifra,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
C. Cocha Toapaxi,
V. Coco,
J. Cogan,
E. Cogneras,
L. Cojocariu,
S.  Collaviti,
P. Collins,
T. Colombo,
M. Colonna,
A. Comerma-Montells,
L. Congedo,
A. Contu,
N. Cooke,
I. Corredoira ,
A. Correia,
G. Corti,
J. Cottee Meldrum,
B. Couturier,
D.C. Craik,
M. Cruz Torres,
E. Curras Rivera,
R. Currie,
C.L. Da Silva,
S. Dadabaev,
L. Dai,
X. Dai,
E. Dall'Occo,
J. Dalseno,
C. D'Ambrosio,
J. Daniel,
A. Danilina,
P. d'Argent,
G. Darze,
A.  Davidson,
J.E. Davies,
O. De Aguiar Francisco,
C. De Angelis,
F. De Benedetti,
J. de Boer,
K. De Bruyn,
S. De Capua,
M. De Cian,
U. De Freitas Carneiro Da Graca,
E. De Lucia,
J.M. De Miranda,
L. De Paula,
M. De Serio,
P. De Simone,
F. De Vellis,
J.A. de Vries,
F. Debernardis,
D. Decamp,
V. Dedu,
S.  Dekkers,
L. Del Buono,
B. Delaney,
H.-P. Dembinski,
J. Deng,
V. Denysenko,
O. Deschamps,
F. Dettori,
B. Dey,
P. Di Nezza,
I. Diachkov,
S. Didenko,
S. Ding,
L. Dittmann,
V. Dobishuk,
A. D.  Docheva,
C. Dong,
A.M. Donohoe,
F. Dordei,
A.C. dos Reis,
A. D.  Dowling,
W. Duan,
P. Duda,
M.W. Dudek,
L. Dufour,
V. Duk,
P. Durante,
M. M. Duras,
J.M. Durham,
O. D.  Durmus,
A. Dziurda,
A. Dzyuba,
S. Easo,
E. Eckstein,
U. Egede,
A. Egorychev,
V. Egorychev,
S. Eisenhardt,
E. Ejopu,
L. Eklund,
M. Elashri,
J. Ellbracht,
S. Ely,
A. Ene,
J. Eschle,
S. Esen,
T. Evans,
F. Fabiano,
L.N. Falcao,
Y. Fan,
B. Fang,
L. Fantini,
M. Faria,
K.   Farmer,
D. Fazzini,
L. Felkowski,
M. Feng,
M. Feo,
A. Fernandez Casani,
M. Fernandez Gomez,
A.D. Fernez,
F. Ferrari,
F. Ferreira Rodrigues,
M. Ferrillo,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiorini,
M. Firlej,
K.L. Fischer,
D.S. Fitzgerald,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
M. Fontana,
L. F.  Foreman,
R. Forty,
D. Foulds-Holt,
V. Franco Lima,
M. Franco Sevilla,
M. Frank,
E. Franzoso,
G. Frau,
C. Frei,
D.A. Friday,
J. Fu,
Q. F{\"u}hring,
Y. Fujii,
T. Fulghesu,
E. Gabriel,
G. Galati,
M.D. Galati,
A. Gallas Torreira,
D. Galli,
S. Gambetta,
M. Gandelman,
P. Gandini,
B.  Ganie,
H. Gao,
R. Gao,
T.Q. Gao,
Y. Gao,
Y. Gao,
Y. Gao,
L.M. Garcia Martin,
P. Garcia Moreno,
J. Garc{\'\i}a Pardi{\~n}as,
P.  Gardner,
K. G.  Garg,
L. Garrido,
C. Gaspar,
A.  Gavrikov,
L.L. Gerken,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
S. Ghizzo,
Z. Ghorbanimoghaddam,
L. Giambastiani,
F. I. Giasemis,
V. Gibson,
H.K. Giemza,
A.L. Gilman,
M. Giovannetti,
A. Giovent{\`u},
L. Girardey,
C. Giugliano,
M.A. Giza,
F.C. Glaser,
V.V. Gligorov,
C. G{\"o}bel,
L.  Golinka-Bezshyyko,
E. Golobardes,
D. Golubkov,
A. Golutvin,
S. Gomez Fernandez,
W.  Gomulka,
F. Goncalves Abrantes,
M. Goncerz,
G. Gong,
J. A. Gooding,
I.V. Gorelov,
C. Gotti,
E. Govorkova,
J.P. Grabowski,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
L. Grazette,
G. Graziani,
A. T. Grecu,
L.M. Greeven,
N.A. Grieser,
L. Grillo,
S. Gromov,
C.  Gu,
M. Guarise,
L.  Guerry,
V. Guliaeva,
P. A. G{\"u}nther,
A.-K. Guseinov,
E. Gushchin,
Y. Guz,
T. Gys,
K. Habermann,
T. Hadavizadeh,
C. Hadjivasiliou,
G. Haefeli,
C. Haen,
G.  Hallett,
M.M. Halvorsen,
P.M. Hamilton,
J. Hammerich,
Q. Han,
X. Han,
S. Hansmann-Menzemer,
L. Hao,
N. Harnew,
T. H.  Harris,
M. Hartmann,
S. Hashmi,
J. He,
F. Hemmer,
C. Henderson,
R.D.L. Henderson,
A.M. Hennequin,
K. Hennessy,
L. Henry,
J. Herd,
P. Herrero Gascon,
J. Heuel,
A. Hicheur,
G. Hijano Mendizabal,
J. Horswill,
R. Hou,
Y. Hou,
N. Howarth,
J. Hu,
W. Hu,
X. Hu,
W. Huang,
W. Hulsbergen,
R.J. Hunter,
M. Hushchyn,
D. Hutchcroft,
M. Idzik,
D. Ilin,
P. Ilten,
A. Inglessi,
A. Iniukhin,
A. Ishteev,
K. Ivshin,
R. Jacobsson,
H. Jage,
S.J. Jaimes Elles,
S. Jakobsen,
E. Jans,
B.K. Jashal,
A. Jawahery,
V. Jevtic,
E. Jiang,
X. Jiang,
Y. Jiang,
Y. J.  Jiang,
M. John,
A.  John Rubesh Rajan,
D. Johnson,
C.R. Jones,
T.P. Jones,
S. Joshi,
B. Jost,
J.  Juan Castella,
N. Jurik,
I. Juszczak,
D. Kaminaris,
S. Kandybei,
M.  Kane,
Y. Kang,
C. Kar,
M. Karacson,
D. Karpenkov,
A. Kauniskangas,
J.W. Kautz,
M.K. Kazanecki,
F. Keizer,
M. Kenzie,
T. Ketel,
B. Khanji,
A. Kharisova,
S. Kholodenko,
G. Khreich,
T. Kirn,
V.S. Kirsebom,
O. Kitouni,
S. Klaver,
N. Kleijne,
K. Klimaszewski,
M.R. Kmiec,
S. Koliiev,
L. Kolk,
A. Konoplyannikov,
P. Kopciewicz,
P. Koppenburg,
M. Korolev,
I. Kostiuk,
O. Kot,
S. Kotriakhova,
A. Kozachuk,
P. Kravchenko,
L. Kravchuk,
M. Kreps,
P. Krokovny,
W. Krupa,
W. Krzemien,
O. Kshyvanskyi,
S. Kubis,
M. Kucharczyk,
V. Kudryavtsev,
E. Kulikova,
A. Kupsc,
B. K.  Kutsenko,
D. Lacarrere,
P.  Laguarta Gonzalez,
A. Lai,
A. Lampis,
D. Lancierini,
C. Landesa Gomez,
J.J. Lane,
R. Lane,
G. Lanfranchi,
C. Langenbruch,
J. Langer,
O. Lantwin,
T. Latham,
F. Lazzari,
C. Lazzeroni,
R. Le Gac,
H.  Lee,
R. Lef{\`e}vre,
A. Leflat,
S. Legotin,
M. Lehuraux,
E. Lemos Cid,
O. Leroy,
T. Lesiak,
E. D. Lesser,
B. Leverington,
A. Li,
C.  Li,
C.  Li,
H. Li,
K. Li,
L. Li,
M. Li,
P. Li,
P.-R. Li,
Q.  Li,
S. Li,
T. Li,
T. Li,
Y. Li,
Y. Li,
Z. Lian,
X. Liang,
S. Libralon,
C. Lin,
T. Lin,
R. Lindner,
H.  Linton,
V. Lisovskyi,
R. Litvinov,
F. L.  Liu,
G. Liu,
K. Liu,
S. Liu,
W.  Liu,
Y. Liu,
Y. Liu,
Y. L.  Liu,
G. Loachamin Ordonez,
A. Lobo Salvia,
A. Loi,
T. Long,
J.H. Lopes,
A. Lopez Huertas,
S. L{\'o}pez Soli{\~n}o,
Q. Lu,
C. Lucarelli,
D. Lucchesi,
M. Lucio Martinez,
V. Lukashenko,
Y. Luo,
A. Lupato,
E. Luppi,
K. Lynch,
X.-R. Lyu,
G. M.  Ma,
S. Maccolini,
F. Machefert,
F. Maciuc,
B.  Mack,
I. Mackay,
L. M.  Mackey,
L.R. Madhan Mohan,
M. J.  Madurai,
A. Maevskiy,
D. Magdalinski,
D. Maisuzenko,
J.J. Malczewski,
S. Malde,
L. Malentacca,
A. Malinin,
T. Maltsev,
G. Manca,
G. Mancinelli,
C. Mancuso,
R. Manera Escalero,
F. M.  Manganella,
D. Manuzzi,
D. Marangotto,
J.F. Marchand,
R. Marchevski,
U. Marconi,
E. Mariani,
S. Mariani,
C. Marin Benito,
J. Marks,
A.M. Marshall,
L.  Martel,
G. Martelli,
G. Martellotti,
L. Martinazzoli,
M. Martinelli,
D.  Martinez Gomez,
D. Martinez Santos,
F. Martinez Vidal,
A.  Martorell i Granollers,
A. Massafferri,
R. Matev,
A. Mathad,
V. Matiunin,
C. Matteuzzi,
K.R. Mattioli,
A. Mauri,
E. Maurice,
J. Mauricio,
P. Mayencourt,
J. Mazorra de Cos,
M. Mazurek,
M. McCann,
T.H. McGrath,
N.T. McHugh,
A. McNab,
R. McNulty,
B. Meadows,
G. Meier,
D. Melnychuk,
F. M.  Meng,
M. Merk,
A. Merli,
L. Meyer Garcia,
D. Miao,
H. Miao,
M. Mikhasenko,
D.A. Milanes,
A. Minotti,
E. Minucci,
T. Miralles,
B. Mitreska,
D.S. Mitzel,
A. Modak,
L. Moeser,
R.A. Mohammed,
R.D. Moise,
S. Mokhnenko,
E. F. Molina Cardenas,
T. Momb{\"a}cher,
M. Monk,
S. Monteil,
A. Morcillo Gomez,
G. Morello,
M.J. Morello,
M.P. Morgenthaler,
J. Moron,
W.  Morren,
A.B. Morris,
A.G. Morris,
R. Mountain,
H. Mu,
Z. M.  Mu,
E. Muhammad,
F. Muheim,
M. Mulder,
K. M{\"u}ller,
F. Mu{\~n}oz-Rojas,
R. Murta,
P. Naik,
T. Nakada,
R. Nandakumar,
T. Nanut,
I. Nasteva,
M. Needham,
N. Neri,
S. Neubert,
N. Neufeld,
P. Neustroev,
J. Nicolini,
D. Nicotra,
E.M. Niel,
N. Nikitin,
Q. Niu,
P. Nogarolli,
P. Nogga,
C. Normand,
J. Novoa Fernandez,
G. Nowak,
C. Nunez,
H. N.  Nur,
A. Oblakowska-Mucha,
V. Obraztsov,
T. Oeser,
S. Okamura,
A. Okhotnikov,
O. Okhrimenko,
R. Oldeman,
F. Oliva,
M. Olocco,
C.J.G. Onderwater,
R.H. O'Neil,
D. Osthues,
J.M. Otalora Goicochea,
P. Owen,
A. Oyanguren,
O. Ozcelik,
F. Paciolla,
A.  Padee,
K.O. Padeken,
B. Pagare,
P.R. Pais,
T. Pajero,
A. Palano,
M. Palutan,
X.  Pan,
G. Panshin,
L. Paolucci,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
C. Pappenheimer,
C. Parkes,
D.  Parmar,
B. Passalacqua,
G. Passaleva,
D. Passaro,
A. Pastore,
M. Patel,
J. Patoc,
C. Patrignani,
A.  Paul,
C.J. Pawley,
A. Pellegrino,
J.  Peng,
M. Pepe Altarelli,
S. Perazzini,
D. Pereima,
H.  Pereira Da Costa,
A. Pereiro Castro,
P. Perret,
A.  Perrevoort,
A. Perro,
M.J. Peters,
K. Petridis,
A. Petrolini,
J. P.  Pfaller,
H. Pham,
L. Pica,
M. Piccini,
L.  Piccolo,
B. Pietrzyk,
G. Pietrzyk,
R. N. Pilato,
D. Pinci,
F. Pisani,
M. Pizzichemi,
V. Placinta,
M. Plo Casasus,
T. Poeschl,
F. Polci,
M. Poli Lener,
A. Poluektov,
N. Polukhina,
I. Polyakov,
E. Polycarpo,
S. Ponce,
D. Popov,
S. Poslavskii,
K. Prasanth,
C. Prouve,
D. Provenzano,
V. Pugatch,
G. Punzi,
S.  Qasim,
Q. Q.  Qian,
W. Qian,
N. Qin,
S. Qu,
R. Quagliani,
R.I. Rabadan Trejo,
J.H. Rademacker,
M. Rama,
M.  Ram\'{i}rez Garc\'{i}a,
V. Ramos De Oliveira,
M. Ramos Pernas,
M.S. Rangel,
F. Ratnikov,
G. Raven,
M. Rebollo De Miguel,
F. Redi,
J. Reich,
F. Reiss,
Z. Ren,
P.K. Resmi,
M.  Ribalda Galvez,
R. Ribatti,
G. Ricart,
D. Riccardi,
S. Ricciardi,
K. Richardson,
M. Richardson-Slipper,
K. Rinnert,
P. Robbe,
G. Robertson,
E. Rodrigues,
A. Rodriguez Alvarez,
E. Rodriguez Fernandez,
J.A. Rodriguez Lopez,
E. Rodriguez Rodriguez,
J. Roensch,
A. Rogachev,
A. Rogovskiy,
D.L. Rolf,
P. Roloff,
V. Romanovskiy,
A. Romero Vidal,
G. Romolini,
F. Ronchetti,
T. Rong,
M. Rotondo,
S. R.  Roy,
M.S. Rudolph,
M. Ruiz Diaz,
R.A. Ruiz Fernandez,
J. Ruiz Vidal,
J. Ryzka,
J. J. Saavedra-Arias,
J.J. Saborido Silva,
R. Sadek,
N. Sagidova,
D. Sahoo,
N. Sahoo,
B. Saitta,
M. Salomoni,
I. Sanderswood,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
L. Santoro ,
E. Santovetti,
A. Saputi,
D. Saranin,
A. Sarnatskiy,
G. Sarpis,
M. Sarpis,
C. Satriano,
A. Satta,
M. Saur,
D. Savrina,
H. Sazak,
F. Sborzacchi,
L.G. Scantlebury Smead,
A. Scarabotto,
S. Schael,
S. Scherl,
M. Schiller,
H. Schindler,
M. Schmelling,
B. Schmidt,
S. Schmitt,
H. Schmitz,
O. Schneider,
A. Schopper,
N. Schulte,
S. Schulte,
M.H. Schune,
R. Schwemmer,
G. Schwering,
B. Sciascia,
A. Sciuccati,
I. Segal,
S. Sellam,
A. Semennikov,
T. Senger,
M. Senghi Soares,
A. Sergi,
N. Serra,
L. Sestini,
A. Seuthe,
Y. Shang,
D.M. Shangase,
M. Shapkin,
R. S.  Sharma,
I. Shchemerov,
L. Shchutska,
T. Shears,
L. Shekhtman,
Z. Shen,
S. Sheng,
V. Shevchenko,
B. Shi,
Q. Shi,
Y. Shimizu,
E. Shmanin,
R. Shorkin,
J.D. Shupperd,
R. Silva Coutinho,
G. Simi,
S. Simone,
N. Skidmore,
T. Skwarnicki,
M.W. Slater,
J.C. Smallwood,
E. Smith,
K. Smith,
M. Smith,
A. Snoch,
L. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
A. Solomin,
A. Solovev,
I. Solovyev,
N. S.  Sommerfeld,
R. Song,
Y. Song,
Y. Song,
Y. S.  Song,
F.L. Souza De Almeida,
B. Souza De Paula,
E. Spadaro Norella,
E. Spedicato,
J.G. Speer,
E. Spiridenkov,
P. Spradlin,
V. Sriskaran,
F. Stagni,
M. Stahl,
S. Stahl,
S. Stanislaus,
M.  Stefaniak,
E.N. Stein,
O. Steinkamp,
O. Stenyakin,
H. Stevens,
D. Strekalina,
Y. Su,
F. Suljik,
J. Sun,
L. Sun,
D. Sundfeld,
W. Sutcliffe,
K. Swientek,
F. Swystun,
A. Szabelski,
T. Szumlak,
Y. Tan,
Y. Tang,
M.D. Tat,
A. Terentev,
F. Terzuoli,
F. Teubert,
E. Thomas,
D.J.D. Thompson,
H. Tilquin,
V. Tisserand,
S. T'Jampens,
M. Tobin,
L. Tomassetti,
G. Tonani,
X. Tong,
T. Tork,
D. Torres Machado,
L. Toscano,
D.Y. Tou,
C. Trippl,
G. Tuci,
N. Tuning,
L.H. Uecker,
A. Ukleja,
D.J. Unverzagt,
B.  Urbach,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
V. Vagnoni,
V.  Valcarce Cadenas,
G. Valenti,
N. Valls Canudas,
J. van Eldik,
H. Van Hecke,
E. van Herwijnen,
C.B. Van Hulse,
R. Van Laak,
M. van Veghel,
G. Vasquez,
R. Vazquez Gomez,
P. Vazquez Regueiro,
C. V{\'a}zquez Sierra,
S. Vecchi,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Verdoglia,
M. Vesterinen,
D.  Vico Benet,
P.  Vidrier Villalba,
M. Vieites Diaz,
X. Vilasis-Cardona,
E. Vilella Figueras,
A. Villa,
P. Vincent,
F.C. Volle,
D. vom Bruch,
N. Voropaev,
K. Vos,
C. Vrahas,
J. Wagner,
J. Walsh,
E.J. Walton,
G. Wan,
C. Wang,
G. Wang,
H. Wang,
J. Wang,
J. Wang,
J. Wang,
J. Wang,
M. Wang,
N. W.  Wang,
R. Wang,
X. Wang,
X. Wang,
X. W.  Wang,
Y. Wang,
Y. W.  Wang,
Z. Wang,
Z. Wang,
Z. Wang,
J.A. Ward,
M. Waterlaat,
N.K. Watson,
D. Websdale,
Y. Wei,
J. Wendel,
B.D.C. Westhenry,
C. White,
M. Whitehead,
E. Whiter,
A.R. Wiederhold,
D. Wiedner,
G. Wilkinson,
M.K. Wilkinson,
M. Williams,
M. J. Williams,
M.R.J. Williams,
R. Williams,
Z.  Williams,
F.F. Wilson,
M. Winn,
W. Wislicki,
M. Witek,
L. Witola,
G. Wormser,
S.A. Wotton,
H. Wu,
J. Wu,
X. Wu,
Y. Wu,
Z. Wu,
K. Wyllie,
S. Xian,
Z. Xiang,
Y. Xie,
T. X.  Xing,
A. Xu,
L. Xu,
L. Xu,
M. Xu,
Z. Xu,
Z. Xu,
Z. Xu,
K.  Yang,
S. Yang,
X. Yang,
Y. Yang,
Z. Yang,
V. Yeroshenko,
H. Yeung,
H. Yin,
X.  Yin,
C. Y.  Yu,
J. Yu,
X. Yuan,
Y Yuan,
E. Zaffaroni,
M. Zavertyaev,
M. Zdybal,
F. Zenesini,
C.  Zeng,
M. Zeng,
C. Zhang,
D. Zhang,
J. Zhang,
L. Zhang,
S. Zhang,
S. Zhang,
Y. Zhang,
Y. Z.  Zhang,
Z. Zhang,
Y. Zhao,
A. Zhelezov,
S. Z.  Zheng,
X. Z.  Zheng,
Y. Zheng,
T. Zhou,
X. Zhou,
Y. Zhou,
V. Zhovkovska,
L. Z.  Zhu,
X. Zhu,
X. Zhu,
V. Zhukov,
J. Zhuo,
Q. Zou,
D. Zuliani,
G. Zunica

==> Authorship_LHCb-PAPER-2024-051.tex <==
% LHCb collaboration author list
% Data extracted on February 6th, 2025 at 12:51pm for paper reference LHCb-PAPER-2024-051
\centerline
{\large\bf LHCb collaboration}
\begin
{flushleft}
\small
R.~Aaij$^{38}$\lhcborcid{0000-0003-0533-1952},
A.S.W.~Abdelmotteleb$^{57}$\lhcborcid{0000-0001-7905-0542},
C.~Abellan~Beteta$^{51}$\lhcborcid{0009-0009-0869-6798},
F.~Abudin{\'e}n$^{57}$\lhcborcid{0000-0002-6737-3528},
T.~Ackernley$^{61}$\lhcborcid{0000-0002-5951-3498},
A. A. ~Adefisoye$^{69}$\lhcborcid{0000-0003-2448-1550},
B.~Adeva$^{47}$\lhcborcid{0000-0001-9756-3712},
M.~Adinolfi$^{55}$\lhcborcid{0000-0002-1326-1264},
P.~Adlarson$^{83}$\lhcborcid{0000-0001-6280-3851},
C.~Agapopoulou$^{14}$\lhcborcid{0000-0002-2368-0147},
C.A.~Aidala$^{85}$\lhcborcid{0000-0001-9540-4988},
Z.~Ajaltouni$^{11}$,
S.~Akar$^{11}$\lhcborcid{0000-0003-0288-9694},
K.~Akiba$^{38}$\lhcborcid{0000-0002-6736-471X},
P.~Albicocco$^{28}$\lhcborcid{0000-0001-6430-1038},
J.~Albrecht$^{19,f}$\lhcborcid{0000-0001-8636-1621},
F.~Alessio$^{49}$\lhcborcid{0000-0001-5317-1098},
M.~Alexander$^{60}$\lhcborcid{0000-0002-8148-2392},
Z.~Aliouche$^{63}$\lhcborcid{0000-0003-0897-4160},
P.~Alvarez~Cartelle$^{56}$\lhcborcid{0000-0003-1652-2834},
R.~Amalric$^{16}$\lhcborcid{0000-0003-4595-2729},
S.~Amato$^{3}$\lhcborcid{0000-0002-3277-0662},
J.L.~Amey$^{55}$\lhcborcid{0000-0002-2597-3808},
Y.~Amhis$^{14}$\lhcborcid{0000-0003-4282-1512},
L.~An$^{6}$\lhcborcid{0000-0002-3274-5627},
L.~Anderlini$^{27}$\lhcborcid{0000-0001-6808-2418},
M.~Andersson$^{51}$\lhcborcid{0000-0003-3594-9163},
A.~Andreianov$^{44}$\lhcborcid{0000-0002-6273-0506},
P.~Andreola$^{51}$\lhcborcid{0000-0002-3923-431X},
M.~Andreotti$^{26}$\lhcborcid{0000-0003-2918-1311},
D.~Andreou$^{69}$\lhcborcid{0000-0001-6288-0558},
A.~Anelli$^{31,o,49}$\lhcborcid{0000-0002-6191-934X},
D.~Ao$^{7}$\lhcborcid{0000-0003-1647-4238},
F.~Archilli$^{37,u}$\lhcborcid{0000-0002-1779-6813},
M.~Argenton$^{26}$\lhcborcid{0009-0006-3169-0077},
S.~Arguedas~Cuendis$^{9,49}$\lhcborcid{0000-0003-4234-7005},
A.~Artamonov$^{44}$\lhcborcid{0000-0002-2785-2233},
M.~Artuso$^{69}$\lhcborcid{0000-0002-5991-7273},
E.~Aslanides$^{13}$\lhcborcid{0000-0003-3286-683X},
R.~Ata\'{i}de~Da~Silva$^{50}$\lhcborcid{0009-0005-1667-2666},
M.~Atzeni$^{65}$\lhcborcid{0000-0002-3208-3336},
B.~Audurier$^{12}$\lhcborcid{0000-0001-9090-4254},
D.~Bacher$^{64}$\lhcborcid{0000-0002-1249-367X},
I.~Bachiller~Perea$^{10}$\lhcborcid{0000-0002-3721-4876},
S.~Bachmann$^{22}$\lhcborcid{0000-0002-1186-3894},
M.~Bachmayer$^{50}$\lhcborcid{0000-0001-5996-2747},
J.J.~Back$^{57}$\lhcborcid{0000-0001-7791-4490},
P.~Baladron~Rodriguez$^{47}$\lhcborcid{0000-0003-4240-2094},
V.~Balagura$^{15}$\lhcborcid{0000-0002-1611-7188},
A. ~Balboni$^{26}$\lhcborcid{0009-0003-8872-976X},
W.~Baldini$^{26}$\lhcborcid{0000-0001-7658-8777},
L.~Balzani$^{19}$\lhcborcid{0009-0006-5241-1452},
H. ~Bao$^{7}$\lhcborcid{0009-0002-7027-021X},
J.~Baptista~de~Souza~Leite$^{61}$\lhcborcid{0000-0002-4442-5372},
C.~Barbero~Pretel$^{47,12}$\lhcborcid{0009-0001-1805-6219},
M.~Barbetti$^{27}$\lhcborcid{0000-0002-6704-6914},
I. R.~Barbosa$^{70}$\lhcborcid{0000-0002-3226-8672},
R.J.~Barlow$^{63}$\lhcborcid{0000-0002-8295-8612},
M.~Barnyakov$^{25}$\lhcborcid{0009-0000-0102-0482},
S.~Barsuk$^{14}$\lhcborcid{0000-0002-0898-6551},
W.~Barter$^{59}$\lhcborcid{0000-0002-9264-4799},
J.~Bartz$^{69}$\lhcborcid{0000-0002-2646-4124},
J.M.~Basels$^{17}$\lhcborcid{0000-0001-5860-8770},
S.~Bashir$^{40}$\lhcborcid{0000-0001-9861-8922},
G.~Bassi$^{35,r}$\lhcborcid{0000-0002-2145-3805},
B.~Batsukh$^{5}$\lhcborcid{0000-0003-1020-2549},
P. B. ~Battista$^{14}$\lhcborcid{0009-0005-5095-0439},
A.~Bay$^{50}$\lhcborcid{0000-0002-4862-9399},
A.~Beck$^{65}$\lhcborcid{0000-0003-4872-1213},
M.~Becker$^{19}$\lhcborcid{0000-0002-7972-8760},
F.~Bedeschi$^{35}$\lhcborcid{0000-0002-8315-2119},
I.B.~Bediaga$^{2}$\lhcborcid{0000-0001-7806-5283},
N. A. ~Behling$^{19}$\lhcborcid{0000-0003-4750-7872},
S.~Belin$^{47}$\lhcborcid{0000-0001-7154-1304},
K.~Belous$^{44}$\lhcborcid{0000-0003-0014-2589},
I.~Belov$^{29}$\lhcborcid{0000-0003-1699-9202},
I.~Belyaev$^{36}$\lhcborcid{0000-0002-7458-7030},
G.~Benane$^{13}$\lhcborcid{0000-0002-8176-8315},
G.~Bencivenni$^{28}$\lhcborcid{0000-0002-5107-0610},
E.~Ben-Haim$^{16}$\lhcborcid{0000-0002-9510-8414},
A.~Berezhnoy$^{44}$\lhcborcid{0000-0002-4431-7582},
R.~Bernet$^{51}$\lhcborcid{0000-0002-4856-8063},
S.~Bernet~Andres$^{45}$\lhcborcid{0000-0002-4515-7541},
A.~Bertolin$^{33}$\lhcborcid{0000-0003-1393-4315},
C.~Betancourt$^{51}$\lhcborcid{0000-0001-9886-7427},
F.~Betti$^{59}$\lhcborcid{0000-0002-2395-235X},
J. ~Bex$^{56}$\lhcborcid{0000-0002-2856-8074},
Ia.~Bezshyiko$^{51}$\lhcborcid{0000-0002-4315-6414},
J.~Bhom$^{41}$\lhcborcid{0000-0002-9709-903X},
M.S.~Bieker$^{19}$\lhcborcid{0000-0001-7113-7862},
N.V.~Biesuz$^{26}$\lhcborcid{0000-0003-3004-0946},
P.~Billoir$^{16}$\lhcborcid{0000-0001-5433-9876},
A.~Biolchini$^{38}$\lhcborcid{0000-0001-6064-9993},
M.~Birch$^{62}$\lhcborcid{0000-0001-9157-4461},
F.C.R.~Bishop$^{10}$\lhcborcid{0000-0002-0023-3897},
A.~Bitadze$^{63}$\lhcborcid{0000-0001-7979-1092},
A.~Bizzeti$^{}$\lhcborcid{0000-0001-5729-5530},
T.~Blake$^{57}$\lhcborcid{0000-0002-0259-5891},
F.~Blanc$^{50}$\lhcborcid{0000-0001-5775-3132},
J.E.~Blank$^{19}$\lhcborcid{0000-0002-6546-5605},
S.~Blusk$^{69}$\lhcborcid{0000-0001-9170-684X},
V.~Bocharnikov$^{44}$\lhcborcid{0000-0003-1048-7732},
J.A.~Boelhauve$^{19}$\lhcborcid{0000-0002-3543-9959},
O.~Boente~Garcia$^{15}$\lhcborcid{0000-0003-0261-8085},
T.~Boettcher$^{66}$\lhcborcid{0000-0002-2439-9955},
A. ~Bohare$^{59}$\lhcborcid{0000-0003-1077-8046},
A.~Boldyrev$^{44}$\lhcborcid{0000-0002-7872-6819},
C.S.~Bolognani$^{80}$\lhcborcid{0000-0003-3752-6789},
R.~Bolzonella$^{26,l}$\lhcborcid{0000-0002-0055-0577},
R. B. ~Bonacci$^{1}$\lhcborcid{0009-0004-1871-2417},
N.~Bondar$^{44}$\lhcborcid{0000-0003-2714-9879},
A.~Bordelius$^{49}$\lhcborcid{0009-0002-3529-8524},
F.~Borgato$^{33}$\lhcborcid{0000-0002-3149-6710},
S.~Borghi$^{63}$\lhcborcid{0000-0001-5135-1511},
M.~Borsato$^{31,o}$\lhcborcid{0000-0001-5760-2924},
J.T.~Borsuk$^{41}$\lhcborcid{0000-0002-9065-9030},
E. ~Bottalico$^{61}$\lhcborcid{0000-0003-2238-8803},
S.A.~Bouchiba$^{50}$\lhcborcid{0000-0002-0044-6470},
M. ~Bovill$^{64}$\lhcborcid{0009-0006-2494-8287},
T.J.V.~Bowcock$^{61}$\lhcborcid{0000-0002-3505-6915},
A.~Boyer$^{49}$\lhcborcid{0000-0002-9909-0186},
C.~Bozzi$^{26}$\lhcborcid{0000-0001-6782-3982},
J. D.~Brandenburg$^{86}$\lhcborcid{0000-0002-6327-5947},
A.~Brea~Rodriguez$^{50}$\lhcborcid{0000-0001-5650-445X},
N.~Breer$^{19}$\lhcborcid{0000-0003-0307-3662},
J.~Brodzicka$^{41}$\lhcborcid{0000-0002-8556-0597},
A.~Brossa~Gonzalo$^{47,\dagger}$\lhcborcid{0000-0002-4442-1048},
J.~Brown$^{61}$\lhcborcid{0000-0001-9846-9672},
D.~Brundu$^{32}$\lhcborcid{0000-0003-4457-5896},
E.~Buchanan$^{59}$\lhcborcid{0009-0008-3263-1823},
L.~Buonincontri$^{33,p}$\lhcborcid{0000-0002-1480-454X},
M. ~Burgos~Marcos$^{80}$\lhcborcid{0009-0001-9716-0793},
A.T.~Burke$^{63}$\lhcborcid{0000-0003-0243-0517},
C.~Burr$^{49}$\lhcborcid{0000-0002-5155-1094},
J.S.~Butter$^{56}$\lhcborcid{0000-0002-1816-536X},
J.~Buytaert$^{49}$\lhcborcid{0000-0002-7958-6790},
W.~Byczynski$^{49}$\lhcborcid{0009-0008-0187-3395},
S.~Cadeddu$^{32}$\lhcborcid{0000-0002-7763-500X},
H.~Cai$^{74}$,
A.~Caillet$^{16}$\lhcborcid{0009-0001-8340-3870},
R.~Calabrese$^{26,l}$\lhcborcid{0000-0002-1354-5400},
S.~Calderon~Ramirez$^{9}$\lhcborcid{0000-0001-9993-4388},
L.~Calefice$^{46}$\lhcborcid{0000-0001-6401-1583},
S.~Cali$^{28}$\lhcborcid{0000-0001-9056-0711},
M.~Calvi$^{31,o}$\lhcborcid{0000-0002-8797-1357},
M.~Calvo~Gomez$^{45}$\lhcborcid{0000-0001-5588-1448},
P.~Camargo~Magalhaes$^{2,z}$\lhcborcid{0000-0003-3641-8110},
J. I.~Cambon~Bouzas$^{47}$\lhcborcid{0000-0002-2952-3118},
P.~Campana$^{28}$\lhcborcid{0000-0001-8233-1951},
D.H.~Campora~Perez$^{80}$\lhcborcid{0000-0001-8998-9975},
A.F.~Campoverde~Quezada$^{7}$\lhcborcid{0000-0003-1968-1216},
S.~Capelli$^{31}$\lhcborcid{0000-0002-8444-4498},
L.~Capriotti$^{26}$\lhcborcid{0000-0003-4899-0587},
R.~Caravaca-Mora$^{9}$\lhcborcid{0000-0001-8010-0447},
A.~Carbone$^{25,j}$\lhcborcid{0000-0002-7045-2243},
L.~Carcedo~Salgado$^{47}$\lhcborcid{0000-0003-3101-3528},
R.~Cardinale$^{29,m}$\lhcborcid{0000-0002-7835-7638},
A.~Cardini$^{32}$\lhcborcid{0000-0002-6649-0298},
P.~Carniti$^{31,o}$\lhcborcid{0000-0002-7820-2732},
L.~Carus$^{22}$\lhcborcid{0009-0009-5251-2474},
A.~Casais~Vidal$^{65}$\lhcborcid{0000-0003-0469-2588},
R.~Caspary$^{22}$\lhcborcid{0000-0002-1449-1619},
G.~Casse$^{61}$\lhcborcid{0000-0002-8516-237X},
M.~Cattaneo$^{49}$\lhcborcid{0000-0001-7707-169X},
G.~Cavallero$^{26,49}$\lhcborcid{0000-0002-8342-7047},
V.~Cavallini$^{26,l}$\lhcborcid{0000-0001-7601-129X},
S.~Celani$^{22}$\lhcborcid{0000-0003-4715-7622},
S. ~Cesare$^{30,n}$\lhcborcid{0000-0003-0886-7111},
A.J.~Chadwick$^{61}$\lhcborcid{0000-0003-3537-9404},
I.~Chahrour$^{85}$\lhcborcid{0000-0002-1472-0987},
H. ~Chang$^{4,b}$\lhcborcid{0009-0002-8662-1918},
M.~Charles$^{16}$\lhcborcid{0000-0003-4795-498X},
Ph.~Charpentier$^{49}$\lhcborcid{0000-0001-9295-8635},
E. ~Chatzianagnostou$^{38}$\lhcborcid{0009-0009-3781-1820},
M.~Chefdeville$^{10}$\lhcborcid{0000-0002-6553-6493},
C.~Chen$^{13}$\lhcborcid{0000-0002-3400-5489},
S.~Chen$^{5}$\lhcborcid{0000-0002-8647-1828},
Z.~Chen$^{7}$\lhcborcid{0000-0002-0215-7269},
A.~Chernov$^{41}$\lhcborcid{0000-0003-0232-6808},
S.~Chernyshenko$^{53}$\lhcborcid{0000-0002-2546-6080},
X. ~Chiotopoulos$^{80}$\lhcborcid{0009-0006-5762-6559},
V.~Chobanova$^{82}$\lhcborcid{0000-0002-1353-6002},
M.~Chrzaszcz$^{41}$\lhcborcid{0000-0001-7901-8710},
A.~Chubykin$^{44}$\lhcborcid{0000-0003-1061-9643},
V.~Chulikov$^{28,36}$\lhcborcid{0000-0002-7767-9117},
P.~Ciambrone$^{28}$\lhcborcid{0000-0003-0253-9846},
X.~Cid~Vidal$^{47}$\lhcborcid{0000-0002-0468-541X},
G.~Ciezarek$^{49}$\lhcborcid{0000-0003-1002-8368},
P.~Cifra$^{49}$\lhcborcid{0000-0003-3068-7029},
P.E.L.~Clarke$^{59}$\lhcborcid{0000-0003-3746-0732},
M.~Clemencic$^{49}$\lhcborcid{0000-0003-1710-6824},
H.V.~Cliff$^{56}$\lhcborcid{0000-0003-0531-0916},
J.~Closier$^{49}$\lhcborcid{0000-0002-0228-9130},
C.~Cocha~Toapaxi$^{22}$\lhcborcid{0000-0001-5812-8611},
V.~Coco$^{49}$\lhcborcid{0000-0002-5310-6808},
J.~Cogan$^{13}$\lhcborcid{0000-0001-7194-7566},
E.~Cogneras$^{11}$\lhcborcid{0000-0002-8933-9427},
L.~Cojocariu$^{43}$\lhcborcid{0000-0002-1281-5923},
S. ~Collaviti$^{50}$\lhcborcid{0009-0003-7280-8236},
P.~Collins$^{49}$\lhcborcid{0000-0003-1437-4022},
T.~Colombo$^{49}$\lhcborcid{0000-0002-9617-9687},
M.~Colonna$^{19}$\lhcborcid{0009-0000-1704-4139},
A.~Comerma-Montells$^{46}$\lhcborcid{0000-0002-8980-6048},
L.~Congedo$^{24}$\lhcborcid{0000-0003-4536-4644},
A.~Contu$^{32}$\lhcborcid{0000-0002-3545-2969},
N.~Cooke$^{60}$\lhcborcid{0000-0002-4179-3700},
I.~Corredoira~$^{47}$\lhcborcid{0000-0002-6089-0899},
A.~Correia$^{16}$\lhcborcid{0000-0002-6483-8596},
G.~Corti$^{49}$\lhcborcid{0000-0003-2857-4471},
J.~Cottee~Meldrum$^{55}$\lhcborcid{0009-0009-3900-6905},
B.~Couturier$^{49}$\lhcborcid{0000-0001-6749-1033},
D.C.~Craik$^{51}$\lhcborcid{0000-0002-3684-1560},
M.~Cruz~Torres$^{2,g}$\lhcborcid{0000-0003-2607-131X},
E.~Curras~Rivera$^{50}$\lhcborcid{0000-0002-6555-0340},
R.~Currie$^{59}$\lhcborcid{0000-0002-0166-9529},
C.L.~Da~Silva$^{68}$\lhcborcid{0000-0003-4106-8258},
S.~Dadabaev$^{44}$\lhcborcid{0000-0002-0093-3244},
L.~Dai$^{71}$\lhcborcid{0000-0002-4070-4729},
X.~Dai$^{4}$\lhcborcid{0000-0003-3395-7151},
E.~Dall'Occo$^{49}$\lhcborcid{0000-0001-9313-4021},
J.~Dalseno$^{47}$\lhcborcid{0000-0003-3288-4683},
C.~D'Ambrosio$^{49}$\lhcborcid{0000-0003-4344-9994},
J.~Daniel$^{11}$\lhcborcid{0000-0002-9022-4264},
A.~Danilina$^{44}$\lhcborcid{0000-0003-3121-2164},
P.~d'Argent$^{24}$\lhcborcid{0000-0003-2380-8355},
G.~Darze$^{3}$\lhcborcid{0000-0002-7666-6533},
A. ~Davidson$^{57}$\lhcborcid{0009-0002-0647-2028},
J.E.~Davies$^{63}$\lhcborcid{0000-0002-5382-8683},
O.~De~Aguiar~Francisco$^{63}$\lhcborcid{0000-0003-2735-678X},
C.~De~Angelis$^{32,k}$\lhcborcid{0009-0005-5033-5866},
F.~De~Benedetti$^{49}$\lhcborcid{0000-0002-7960-3116},
J.~de~Boer$^{38}$\lhcborcid{0000-0002-6084-4294},
K.~De~Bruyn$^{79}$\lhcborcid{0000-0002-0615-4399},
S.~De~Capua$^{63}$\lhcborcid{0000-0002-6285-9596},
M.~De~Cian$^{22}$\lhcborcid{0000-0002-1268-9621},
U.~De~Freitas~Carneiro~Da~Graca$^{2,a}$\lhcborcid{0000-0003-0451-4028},
E.~De~Lucia$^{28}$\lhcborcid{0000-0003-0793-0844},
J.M.~De~Miranda$^{2}$\lhcborcid{0009-0003-2505-7337},
L.~De~Paula$^{3}$\lhcborcid{0000-0002-4984-7734},
M.~De~Serio$^{24,h}$\lhcborcid{0000-0003-4915-7933},
P.~De~Simone$^{28}$\lhcborcid{0000-0001-9392-2079},
F.~De~Vellis$^{19}$\lhcborcid{0000-0001-7596-5091},
J.A.~de~Vries$^{80}$\lhcborcid{0000-0003-4712-9816},
F.~Debernardis$^{24}$\lhcborcid{0009-0001-5383-4899},
D.~Decamp$^{10}$\lhcborcid{0000-0001-9643-6762},
V.~Dedu$^{13}$\lhcborcid{0000-0001-5672-8672},
S. ~Dekkers$^{1}$\lhcborcid{0000-0001-9598-875X},
L.~Del~Buono$^{16}$\lhcborcid{0000-0003-4774-2194},
B.~Delaney$^{65}$\lhcborcid{0009-0007-6371-8035},
H.-P.~Dembinski$^{19}$\lhcborcid{0000-0003-3337-3850},
J.~Deng$^{8}$\lhcborcid{0000-0002-4395-3616},
V.~Denysenko$^{51}$\lhcborcid{0000-0002-0455-5404},
O.~Deschamps$^{11}$\lhcborcid{0000-0002-7047-6042},
F.~Dettori$^{32,k}$\lhcborcid{0000-0003-0256-8663},
B.~Dey$^{77}$\lhcborcid{0000-0002-4563-5806},
P.~Di~Nezza$^{28}$\lhcborcid{0000-0003-4894-6762},
I.~Diachkov$^{44}$\lhcborcid{0000-0001-5222-5293},
S.~Didenko$^{44}$\lhcborcid{0000-0001-5671-5863},
S.~Ding$^{69}$\lhcborcid{0000-0002-5946-581X},
L.~Dittmann$^{22}$\lhcborcid{0009-0000-0510-0252},
V.~Dobishuk$^{53}$\lhcborcid{0000-0001-9004-3255},
A. D. ~Docheva$^{60}$\lhcborcid{0000-0002-7680-4043},
C.~Dong$^{4,b}$\lhcborcid{0000-0003-3259-6323},
A.M.~Donohoe$^{23}$\lhcborcid{0000-0002-4438-3950},
F.~Dordei$^{32}$\lhcborcid{0000-0002-2571-5067},
A.C.~dos~Reis$^{2}$\lhcborcid{0000-0001-7517-8418},
A. D. ~Dowling$^{69}$\lhcborcid{0009-0007-1406-3343},
W.~Duan$^{72}$\lhcborcid{0000-0003-1765-9939},
P.~Duda$^{81}$\lhcborcid{0000-0003-4043-7963},
M.W.~Dudek$^{41}$\lhcborcid{0000-0003-3939-3262},
L.~Dufour$^{49}$\lhcborcid{0000-0002-3924-2774},
V.~Duk$^{34}$\lhcborcid{0000-0001-6440-0087},
P.~Durante$^{49}$\lhcborcid{0000-0002-1204-2270},
M. M.~Duras$^{81}$\lhcborcid{0000-0002-4153-5293},
J.M.~Durham$^{68}$\lhcborcid{0000-0002-5831-3398},
O. D. ~Durmus$^{77}$\lhcborcid{0000-0002-8161-7832},
A.~Dziurda$^{41}$\lhcborcid{0000-0003-4338-7156},
A.~Dzyuba$^{44}$\lhcborcid{0000-0003-3612-3195},
S.~Easo$^{58}$\lhcborcid{0000-0002-4027-7333},
E.~Eckstein$^{18}$\lhcborcid{0009-0009-5267-5177},
U.~Egede$^{1}$\lhcborcid{0000-0001-5493-0762},
A.~Egorychev$^{44}$\lhcborcid{0000-0001-5555-8982},
V.~Egorychev$^{44}$\lhcborcid{0000-0002-2539-673X},
S.~Eisenhardt$^{59}$\lhcborcid{0000-0002-4860-6779},
E.~Ejopu$^{63}$\lhcborcid{0000-0003-3711-7547},
L.~Eklund$^{83}$\lhcborcid{0000-0002-2014-3864},
M.~Elashri$^{66}$\lhcborcid{0000-0001-9398-953X},
J.~Ellbracht$^{19}$\lhcborcid{0000-0003-1231-6347},
S.~Ely$^{62}$\lhcborcid{0000-0003-1618-3617},
A.~Ene$^{43}$\lhcborcid{0000-0001-5513-0927},
J.~Eschle$^{69}$\lhcborcid{0000-0002-7312-3699},
S.~Esen$^{22}$\lhcborcid{0000-0003-2437-8078},
T.~Evans$^{63}$\lhcborcid{0000-0003-3016-1879},
F.~Fabiano$^{32}$\lhcborcid{0000-0001-6915-9923},
L.N.~Falcao$^{2}$\lhcborcid{0000-0003-3441-583X},
Y.~Fan$^{7}$\lhcborcid{0000-0002-3153-430X},
B.~Fang$^{7}$\lhcborcid{0000-0003-0030-3813},
L.~Fantini$^{34,q,49}$\lhcborcid{0000-0002-2351-3998},
M.~Faria$^{50}$\lhcborcid{0000-0002-4675-4209},
K.  ~Farmer$^{59}$\lhcborcid{0000-0003-2364-2877},
D.~Fazzini$^{31,o}$\lhcborcid{0000-0002-5938-4286},
L.~Felkowski$^{81}$\lhcborcid{0000-0002-0196-910X},
M.~Feng$^{5,7}$\lhcborcid{0000-0002-6308-5078},
M.~Feo$^{2}$\lhcborcid{0000-0001-5266-2442},
A.~Fernandez~Casani$^{48}$\lhcborcid{0000-0003-1394-509X},
M.~Fernandez~Gomez$^{47}$\lhcborcid{0000-0003-1984-4759},
A.D.~Fernez$^{67}$\lhcborcid{0000-0001-9900-6514},
F.~Ferrari$^{25,j}$\lhcborcid{0000-0002-3721-4585},
F.~Ferreira~Rodrigues$^{3}$\lhcborcid{0000-0002-4274-5583},
M.~Ferrillo$^{51}$\lhcborcid{0000-0003-1052-2198},
M.~Ferro-Luzzi$^{49}$\lhcborcid{0009-0008-1868-2165},
S.~Filippov$^{44}$\lhcborcid{0000-0003-3900-3914},
R.A.~Fini$^{24}$\lhcborcid{0000-0002-3821-3998},
M.~Fiorini$^{26,l}$\lhcborcid{0000-0001-6559-2084},
M.~Firlej$^{40}$\lhcborcid{0000-0002-1084-0084},
K.L.~Fischer$^{64}$\lhcborcid{0009-0000-8700-9910},
D.S.~Fitzgerald$^{85}$\lhcborcid{0000-0001-6862-6876},
C.~Fitzpatrick$^{63}$\lhcborcid{0000-0003-3674-0812},
T.~Fiutowski$^{40}$\lhcborcid{0000-0003-2342-8854},
F.~Fleuret$^{15}$\lhcborcid{0000-0002-2430-782X},
M.~Fontana$^{25}$\lhcborcid{0000-0003-4727-831X},
L. F. ~Foreman$^{63}$\lhcborcid{0000-0002-2741-9966},
R.~Forty$^{49}$\lhcborcid{0000-0003-2103-7577},
D.~Foulds-Holt$^{56}$\lhcborcid{0000-0001-9921-687X},
V.~Franco~Lima$^{3}$\lhcborcid{0000-0002-3761-209X},
M.~Franco~Sevilla$^{67}$\lhcborcid{0000-0002-5250-2948},
M.~Frank$^{49}$\lhcborcid{0000-0002-4625-559X},
E.~Franzoso$^{26,l}$\lhcborcid{0000-0003-2130-1593},
G.~Frau$^{63}$\lhcborcid{0000-0003-3160-482X},
C.~Frei$^{49}$\lhcborcid{0000-0001-5501-5611},
D.A.~Friday$^{63}$\lhcborcid{0000-0001-9400-3322},
J.~Fu$^{7}$\lhcborcid{0000-0003-3177-2700},
Q.~F{\"u}hring$^{19,f,56}$\lhcborcid{0000-0003-3179-2525},
Y.~Fujii$^{1}$\lhcborcid{0000-0002-0813-3065},
T.~Fulghesu$^{16}$\lhcborcid{0000-0001-9391-8619},
E.~Gabriel$^{38}$\lhcborcid{0000-0001-8300-5939},
G.~Galati$^{24}$\lhcborcid{0000-0001-7348-3312},
M.D.~Galati$^{38}$\lhcborcid{0000-0002-8716-4440},
A.~Gallas~Torreira$^{47}$\lhcborcid{0000-0002-2745-7954},
D.~Galli$^{25,j}$\lhcborcid{0000-0003-2375-6030},
S.~Gambetta$^{59}$\lhcborcid{0000-0003-2420-0501},
M.~Gandelman$^{3}$\lhcborcid{0000-0001-8192-8377},
P.~Gandini$^{30}$\lhcborcid{0000-0001-7267-6008},
B. ~Ganie$^{63}$\lhcborcid{0009-0008-7115-3940},
H.~Gao$^{7}$\lhcborcid{0000-0002-6025-6193},
R.~Gao$^{64}$\lhcborcid{0009-0004-1782-7642},
T.Q.~Gao$^{56}$\lhcborcid{0000-0001-7933-0835},
Y.~Gao$^{8}$\lhcborcid{0000-0002-6069-8995},
Y.~Gao$^{6}$\lhcborcid{0000-0003-1484-0943},
Y.~Gao$^{8}$\lhcborcid{0009-0002-5342-4475},
L.M.~Garcia~Martin$^{50}$\lhcborcid{0000-0003-0714-8991},
P.~Garcia~Moreno$^{46}$\lhcborcid{0000-0002-3612-1651},
J.~Garc{\'\i}a~Pardi{\~n}as$^{49}$\lhcborcid{0000-0003-2316-8829},
P. ~Gardner$^{67}$\lhcborcid{0000-0002-8090-563X},
K. G. ~Garg$^{8}$\lhcborcid{0000-0002-8512-8219},
L.~Garrido$^{46}$\lhcborcid{0000-0001-8883-6539},
C.~Gaspar$^{49}$\lhcborcid{0000-0002-8009-1509},
A. ~Gavrikov$^{33}$\lhcborcid{0000-0002-6741-5409},
L.L.~Gerken$^{19}$\lhcborcid{0000-0002-6769-3679},
E.~Gersabeck$^{63}$\lhcborcid{0000-0002-2860-6528},
M.~Gersabeck$^{20}$\lhcborcid{0000-0002-0075-8669},
T.~Gershon$^{57}$\lhcborcid{0000-0002-3183-5065},
S.~Ghizzo$^{29,m}$\lhcborcid{0009-0001-5178-9385},
Z.~Ghorbanimoghaddam$^{55}$\lhcborcid{0000-0002-4410-9505},
L.~Giambastiani$^{33,p}$\lhcborcid{0000-0002-5170-0635},
F. I.~Giasemis$^{16,e}$\lhcborcid{0000-0003-0622-1069},
V.~Gibson$^{56}$\lhcborcid{0000-0002-6661-1192},
H.K.~Giemza$^{42}$\lhcborcid{0000-0003-2597-8796},
A.L.~Gilman$^{64}$\lhcborcid{0000-0001-5934-7541},
M.~Giovannetti$^{28}$\lhcborcid{0000-0003-2135-9568},
A.~Giovent{\`u}$^{46}$\lhcborcid{0000-0001-5399-326X},
L.~Girardey$^{63,58}$\lhcborcid{0000-0002-8254-7274},
C.~Giugliano$^{26,l}$\lhcborcid{0000-0002-6159-4557},
M.A.~Giza$^{41}$\lhcborcid{0000-0002-0805-1561},
F.C.~Glaser$^{14,22}$\lhcborcid{0000-0001-8416-5416},
V.V.~Gligorov$^{16,49}$\lhcborcid{0000-0002-8189-8267},
C.~G{\"o}bel$^{70}$\lhcborcid{0000-0003-0523-495X},
L. ~Golinka-Bezshyyko$^{84}$\lhcborcid{0000-0002-0613-5374},
E.~Golobardes$^{45}$\lhcborcid{0000-0001-8080-0769},
D.~Golubkov$^{44}$\lhcborcid{0000-0001-6216-1596},
A.~Golutvin$^{62,49,44}$\lhcborcid{0000-0003-2500-8247},
S.~Gomez~Fernandez$^{46}$\lhcborcid{0000-0002-3064-9834},
W. ~Gomulka$^{40}$\lhcborcid{0009-0003-2873-425X},
F.~Goncalves~Abrantes$^{64}$\lhcborcid{0000-0002-7318-482X},
M.~Goncerz$^{41}$\lhcborcid{0000-0002-9224-914X},
G.~Gong$^{4,b}$\lhcborcid{0000-0002-7822-3947},
J. A.~Gooding$^{19}$\lhcborcid{0000-0003-3353-9750},
I.V.~Gorelov$^{44}$\lhcborcid{0000-0001-5570-0133},
C.~Gotti$^{31}$\lhcborcid{0000-0003-2501-9608},
E.~Govorkova$^{65}$\lhcborcid{0000-0003-1920-6618},
J.P.~Grabowski$^{18}$\lhcborcid{0000-0001-8461-8382},
L.A.~Granado~Cardoso$^{49}$\lhcborcid{0000-0003-2868-2173},
E.~Graug{\'e}s$^{46}$\lhcborcid{0000-0001-6571-4096},
E.~Graverini$^{50,s}$\lhcborcid{0000-0003-4647-6429},
L.~Grazette$^{57}$\lhcborcid{0000-0001-7907-4261},
G.~Graziani$^{}$\lhcborcid{0000-0001-8212-846X},
A. T.~Grecu$^{43}$\lhcborcid{0000-0002-7770-1839},
L.M.~Greeven$^{38}$\lhcborcid{0000-0001-5813-7972},
N.A.~Grieser$^{66}$\lhcborcid{0000-0003-0386-4923},
L.~Grillo$^{60}$\lhcborcid{0000-0001-5360-0091},
S.~Gromov$^{44}$\lhcborcid{0000-0002-8967-3644},
C. ~Gu$^{15}$\lhcborcid{0000-0001-5635-6063},
M.~Guarise$^{26}$\lhcborcid{0000-0001-8829-9681},
L. ~Guerry$^{11}$\lhcborcid{0009-0004-8932-4024},
V.~Guliaeva$^{44}$\lhcborcid{0000-0003-3676-5040},
P. A.~G{\"u}nther$^{22}$\lhcborcid{0000-0002-4057-4274},
A.-K.~Guseinov$^{50}$\lhcborcid{0000-0002-5115-0581},
E.~Gushchin$^{44}$\lhcborcid{0000-0001-8857-1665},
Y.~Guz$^{6,49,44}$\lhcborcid{0000-0001-7552-400X},
T.~Gys$^{49}$\lhcborcid{0000-0002-6825-6497},
K.~Habermann$^{18}$\lhcborcid{0009-0002-6342-5965},
T.~Hadavizadeh$^{1}$\lhcborcid{0000-0001-5730-8434},
C.~Hadjivasiliou$^{67}$\lhcborcid{0000-0002-2234-0001},
G.~Haefeli$^{50}$\lhcborcid{0000-0002-9257-839X},
C.~Haen$^{49}$\lhcborcid{0000-0002-4947-2928},
G. ~Hallett$^{57}$\lhcborcid{0009-0005-1427-6520},
M.M.~Halvorsen$^{49}$\lhcborcid{0000-0003-0959-3853},
P.M.~Hamilton$^{67}$\lhcborcid{0000-0002-2231-1374},
J.~Hammerich$^{61}$\lhcborcid{0000-0002-5556-1775},
Q.~Han$^{33}$\lhcborcid{0000-0002-7958-2917},
X.~Han$^{22,49}$\lhcborcid{0000-0001-7641-7505},
S.~Hansmann-Menzemer$^{22}$\lhcborcid{0000-0002-3804-8734},
L.~Hao$^{7}$\lhcborcid{0000-0001-8162-4277},
N.~Harnew$^{64}$\lhcborcid{0000-0001-9616-6651},
T. H. ~Harris$^{1}$\lhcborcid{0009-0000-1763-6759},
M.~Hartmann$^{14}$\lhcborcid{0009-0005-8756-0960},
S.~Hashmi$^{40}$\lhcborcid{0000-0003-2714-2706},
J.~He$^{7,c}$\lhcborcid{0000-0002-1465-0077},
F.~Hemmer$^{49}$\lhcborcid{0000-0001-8177-0856},
C.~Henderson$^{66}$\lhcborcid{0000-0002-6986-9404},
R.D.L.~Henderson$^{1,57}$\lhcborcid{0000-0001-6445-4907},
A.M.~Hennequin$^{49}$\lhcborcid{0009-0008-7974-3785},
K.~Hennessy$^{61}$\lhcborcid{0000-0002-1529-8087},
L.~Henry$^{50}$\lhcborcid{0000-0003-3605-832X},
J.~Herd$^{62}$\lhcborcid{0000-0001-7828-3694},
P.~Herrero~Gascon$^{22}$\lhcborcid{0000-0001-6265-8412},
J.~Heuel$^{17}$\lhcborcid{0000-0001-9384-6926},
A.~Hicheur$^{3}$\lhcborcid{0000-0002-3712-7318},
G.~Hijano~Mendizabal$^{51}$\lhcborcid{0009-0002-1307-1759},
J.~Horswill$^{63}$\lhcborcid{0000-0002-9199-8616},
R.~Hou$^{8}$\lhcborcid{0000-0002-3139-3332},
Y.~Hou$^{11}$\lhcborcid{0000-0001-6454-278X},
N.~Howarth$^{61}$\lhcborcid{0009-0001-7370-061X},
J.~Hu$^{72}$\lhcborcid{0000-0002-8227-4544},
W.~Hu$^{6}$\lhcborcid{0000-0002-2855-0544},
X.~Hu$^{4,b}$\lhcborcid{0000-0002-5924-2683},
W.~Huang$^{7}$\lhcborcid{0000-0002-1407-1729},
W.~Hulsbergen$^{38}$\lhcborcid{0000-0003-3018-5707},
R.J.~Hunter$^{57}$\lhcborcid{0000-0001-7894-8799},
M.~Hushchyn$^{44}$\lhcborcid{0000-0002-8894-6292},
D.~Hutchcroft$^{61}$\lhcborcid{0000-0002-4174-6509},
M.~Idzik$^{40}$\lhcborcid{0000-0001-6349-0033},
D.~Ilin$^{44}$\lhcborcid{0000-0001-8771-3115},
P.~Ilten$^{66}$\lhcborcid{0000-0001-5534-1732},
A.~Inglessi$^{44}$\lhcborcid{0000-0002-2522-6722},
A.~Iniukhin$^{44}$\lhcborcid{0000-0002-1940-6276},
A.~Ishteev$^{44}$\lhcborcid{0000-0003-1409-1428},
K.~Ivshin$^{44}$\lhcborcid{0000-0001-8403-0706},
R.~Jacobsson$^{49}$\lhcborcid{0000-0003-4971-7160},
H.~Jage$^{17}$\lhcborcid{0000-0002-8096-3792},
S.J.~Jaimes~Elles$^{75,49,48}$\lhcborcid{0000-0003-0182-8638},
S.~Jakobsen$^{49}$\lhcborcid{0000-0002-6564-040X},
E.~Jans$^{38}$\lhcborcid{0000-0002-5438-9176},
B.K.~Jashal$^{48}$\lhcborcid{0000-0002-0025-4663},
A.~Jawahery$^{67}$\lhcborcid{0000-0003-3719-119X},
V.~Jevtic$^{19,f}$\lhcborcid{0000-0001-6427-4746},
E.~Jiang$^{67}$\lhcborcid{0000-0003-1728-8525},
X.~Jiang$^{5,7}$\lhcborcid{0000-0001-8120-3296},
Y.~Jiang$^{7}$\lhcborcid{0000-0002-8964-5109},
Y. J. ~Jiang$^{6}$\lhcborcid{0000-0002-0656-8647},
M.~John$^{64}$\lhcborcid{0000-0002-8579-844X},
A. ~John~Rubesh~Rajan$^{23}$\lhcborcid{0000-0002-9850-4965},
D.~Johnson$^{54}$\lhcborcid{0000-0003-3272-6001},
C.R.~Jones$^{56}$\lhcborcid{0000-0003-1699-8816},
T.P.~Jones$^{57}$\lhcborcid{0000-0001-5706-7255},
S.~Joshi$^{42}$\lhcborcid{0000-0002-5821-1674},
B.~Jost$^{49}$\lhcborcid{0009-0005-4053-1222},
J. ~Juan~Castella$^{56}$\lhcborcid{0009-0009-5577-1308},
N.~Jurik$^{49}$\lhcborcid{0000-0002-6066-7232},
I.~Juszczak$^{41}$\lhcborcid{0000-0002-1285-3911},
D.~Kaminaris$^{50}$\lhcborcid{0000-0002-8912-4653},
S.~Kandybei$^{52}$\lhcborcid{0000-0003-3598-0427},
M. ~Kane$^{59}$\lhcborcid{ 0009-0006-5064-966X},
Y.~Kang$^{4,b}$\lhcborcid{0000-0002-6528-8178},
C.~Kar$^{11}$\lhcborcid{0000-0002-6407-6974},
M.~Karacson$^{49}$\lhcborcid{0009-0006-1867-9674},
D.~Karpenkov$^{44}$\lhcborcid{0000-0001-8686-2303},
A.~Kauniskangas$^{50}$\lhcborcid{0000-0002-4285-8027},
J.W.~Kautz$^{66}$\lhcborcid{0000-0001-8482-5576},
M.K.~Kazanecki$^{41}$\lhcborcid{0009-0009-3480-5724},
F.~Keizer$^{49}$\lhcborcid{0000-0002-1290-6737},
M.~Kenzie$^{56}$\lhcborcid{0000-0001-7910-4109},
T.~Ketel$^{38}$\lhcborcid{0000-0002-9652-1964},
B.~Khanji$^{69}$\lhcborcid{0000-0003-3838-281X},
A.~Kharisova$^{44}$\lhcborcid{0000-0002-5291-9583},
S.~Kholodenko$^{35,49}$\lhcborcid{0000-0002-0260-6570},
G.~Khreich$^{14}$\lhcborcid{0000-0002-6520-8203},
T.~Kirn$^{17}$\lhcborcid{0000-0002-0253-8619},
V.S.~Kirsebom$^{31,o}$\lhcborcid{0009-0005-4421-9025},
O.~Kitouni$^{65}$\lhcborcid{0000-0001-9695-8165},
S.~Klaver$^{39}$\lhcborcid{0000-0001-7909-1272},
N.~Kleijne$^{35,r}$\lhcborcid{0000-0003-0828-0943},
K.~Klimaszewski$^{42}$\lhcborcid{0000-0003-0741-5922},
M.R.~Kmiec$^{42}$\lhcborcid{0000-0002-1821-1848},
S.~Koliiev$^{53}$\lhcborcid{0009-0002-3680-1224},
L.~Kolk$^{19}$\lhcborcid{0000-0003-2589-5130},
A.~Konoplyannikov$^{44}$\lhcborcid{0009-0005-2645-8364},
P.~Kopciewicz$^{49}$\lhcborcid{0000-0001-9092-3527},
P.~Koppenburg$^{38}$\lhcborcid{0000-0001-8614-7203},
M.~Korolev$^{44}$\lhcborcid{0000-0002-7473-2031},
I.~Kostiuk$^{38}$\lhcborcid{0000-0002-8767-7289},
O.~Kot$^{53}$,
S.~Kotriakhova$^{}$\lhcborcid{0000-0002-1495-0053},
A.~Kozachuk$^{44}$\lhcborcid{0000-0001-6805-0395},
P.~Kravchenko$^{44}$\lhcborcid{0000-0002-4036-2060},
L.~Kravchuk$^{44}$\lhcborcid{0000-0001-8631-4200},
M.~Kreps$^{57}$\lhcborcid{0000-0002-6133-486X},
P.~Krokovny$^{44}$\lhcborcid{0000-0002-1236-4667},
W.~Krupa$^{69}$\lhcborcid{0000-0002-7947-465X},
W.~Krzemien$^{42}$\lhcborcid{0000-0002-9546-358X},
O.~Kshyvanskyi$^{53}$\lhcborcid{0009-0003-6637-841X},
S.~Kubis$^{81}$\lhcborcid{0000-0001-8774-8270},
M.~Kucharczyk$^{41}$\lhcborcid{0000-0003-4688-0050},
V.~Kudryavtsev$^{44}$\lhcborcid{0009-0000-2192-995X},
E.~Kulikova$^{44}$\lhcborcid{0009-0002-8059-5325},
A.~Kupsc$^{83}$\lhcborcid{0000-0003-4937-2270},
B. K. ~Kutsenko$^{13}$\lhcborcid{0000-0002-8366-1167},
D.~Lacarrere$^{49}$\lhcborcid{0009-0005-6974-140X},
P. ~Laguarta~Gonzalez$^{46}$\lhcborcid{0009-0005-3844-0778},
A.~Lai$^{32}$\lhcborcid{0000-0003-1633-0496},
A.~Lampis$^{32}$\lhcborcid{0000-0002-5443-4870},
D.~Lancierini$^{56}$\lhcborcid{0000-0003-1587-4555},
C.~Landesa~Gomez$^{47}$\lhcborcid{0000-0001-5241-8642},
J.J.~Lane$^{1}$\lhcborcid{0000-0002-5816-9488},
R.~Lane$^{55}$\lhcborcid{0000-0002-2360-2392},
G.~Lanfranchi$^{28}$\lhcborcid{0000-0002-9467-8001},
C.~Langenbruch$^{22}$\lhcborcid{0000-0002-3454-7261},
J.~Langer$^{19}$\lhcborcid{0000-0002-0322-5550},
O.~Lantwin$^{44}$\lhcborcid{0000-0003-2384-5973},
T.~Latham$^{57}$\lhcborcid{0000-0002-7195-8537},
F.~Lazzari$^{35,s,49}$\lhcborcid{0000-0002-3151-3453},
C.~Lazzeroni$^{54}$\lhcborcid{0000-0003-4074-4787},
R.~Le~Gac$^{13}$\lhcborcid{0000-0002-7551-6971},
H. ~Lee$^{61}$\lhcborcid{0009-0003-3006-2149},
R.~Lef{\`e}vre$^{11}$\lhcborcid{0000-0002-6917-6210},
A.~Leflat$^{44}$\lhcborcid{0000-0001-9619-6666},
S.~Legotin$^{44}$\lhcborcid{0000-0003-3192-6175},
M.~Lehuraux$^{57}$\lhcborcid{0000-0001-7600-7039},
E.~Lemos~Cid$^{49}$\lhcborcid{0000-0003-3001-6268},
O.~Leroy$^{13}$\lhcborcid{0000-0002-2589-240X},
T.~Lesiak$^{41}$\lhcborcid{0000-0002-3966-2998},
E. D.~Lesser$^{49}$\lhcborcid{0000-0001-8367-8703},
B.~Leverington$^{22}$\lhcborcid{0000-0001-6640-7274},
A.~Li$^{4,b}$\lhcborcid{0000-0001-5012-6013},
C. ~Li$^{4,b}$\lhcborcid{0009-0002-3366-2871},
C. ~Li$^{13}$\lhcborcid{0000-0002-3554-5479},
H.~Li$^{72}$\lhcborcid{0000-0002-2366-9554},
K.~Li$^{8}$\lhcborcid{0000-0002-2243-8412},
L.~Li$^{63}$\lhcborcid{0000-0003-4625-6880},
M.~Li$^{8}$\lhcborcid{0009-0002-3024-1545},
P.~Li$^{7}$\lhcborcid{0000-0003-2740-9765},
P.-R.~Li$^{73}$\lhcborcid{0000-0002-1603-3646},
Q. ~Li$^{5,7}$\lhcborcid{0009-0004-1932-8580},
S.~Li$^{8}$\lhcborcid{0000-0001-5455-3768},
T.~Li$^{5,d}$\lhcborcid{0000-0002-5241-2555},
T.~Li$^{72}$\lhcborcid{0000-0002-5723-0961},
Y.~Li$^{8}$\lhcborcid{0009-0004-0130-6121},
Y.~Li$^{5}$\lhcborcid{0000-0003-2043-4669},
Z.~Lian$^{4,b}$\lhcborcid{0000-0003-4602-6946},
X.~Liang$^{69}$\lhcborcid{0000-0002-5277-9103},
S.~Libralon$^{48}$\lhcborcid{0009-0002-5841-9624},
C.~Lin$^{7}$\lhcborcid{0000-0001-7587-3365},
T.~Lin$^{58}$\lhcborcid{0000-0001-6052-8243},
R.~Lindner$^{49}$\lhcborcid{0000-0002-5541-6500},
H. ~Linton$^{62}$\lhcborcid{0009-0000-3693-1972},
V.~Lisovskyi$^{50}$\lhcborcid{0000-0003-4451-214X},
R.~Litvinov$^{32,49}$\lhcborcid{0000-0002-4234-435X},
F. L. ~Liu$^{1}$\lhcborcid{0009-0002-2387-8150},
G.~Liu$^{72}$\lhcborcid{0000-0001-5961-6588},
K.~Liu$^{73}$\lhcborcid{0000-0003-4529-3356},
S.~Liu$^{5,7}$\lhcborcid{0000-0002-6919-227X},
W. ~Liu$^{8}$\lhcborcid{0009-0005-0734-2753},
Y.~Liu$^{59}$\lhcborcid{0000-0003-3257-9240},
Y.~Liu$^{73}$\lhcborcid{0009-0002-0885-5145},
Y. L. ~Liu$^{62}$\lhcborcid{0000-0001-9617-6067},
G.~Loachamin~Ordonez$^{70}$\lhcborcid{0009-0001-3549-3939},
A.~Lobo~Salvia$^{46}$\lhcborcid{0000-0002-2375-9509},
A.~Loi$^{32}$\lhcborcid{0000-0003-4176-1503},
T.~Long$^{56}$\lhcborcid{0000-0001-7292-848X},
J.H.~Lopes$^{3}$\lhcborcid{0000-0003-1168-9547},
A.~Lopez~Huertas$^{46}$\lhcborcid{0000-0002-6323-5582},
S.~L{\'o}pez~Soli{\~n}o$^{47}$\lhcborcid{0000-0001-9892-5113},
Q.~Lu$^{15}$\lhcborcid{0000-0002-6598-1941},
C.~Lucarelli$^{27}$\lhcborcid{0000-0002-8196-1828},
D.~Lucchesi$^{33,p}$\lhcborcid{0000-0003-4937-7637},
M.~Lucio~Martinez$^{80}$\lhcborcid{0000-0001-6823-2607},
V.~Lukashenko$^{38,53}$\lhcborcid{0000-0002-0630-5185},
Y.~Luo$^{6}$\lhcborcid{0009-0001-8755-2937},
A.~Lupato$^{33,i}$\lhcborcid{0000-0003-0312-3914},
E.~Luppi$^{26,l}$\lhcborcid{0000-0002-1072-5633},
K.~Lynch$^{23}$\lhcborcid{0000-0002-7053-4951},
X.-R.~Lyu$^{7}$\lhcborcid{0000-0001-5689-9578},
G. M. ~Ma$^{4,b}$\lhcborcid{0000-0001-8838-5205},
S.~Maccolini$^{19}$\lhcborcid{0000-0002-9571-7535},
F.~Machefert$^{14}$\lhcborcid{0000-0002-4644-5916},
F.~Maciuc$^{43}$\lhcborcid{0000-0001-6651-9436},
B. ~Mack$^{69}$\lhcborcid{0000-0001-8323-6454},
I.~Mackay$^{64}$\lhcborcid{0000-0003-0171-7890},
L. M. ~Mackey$^{69}$\lhcborcid{0000-0002-8285-3589},
L.R.~Madhan~Mohan$^{56}$\lhcborcid{0000-0002-9390-8821},
M. J. ~Madurai$^{54}$\lhcborcid{0000-0002-6503-0759},
A.~Maevskiy$^{44}$\lhcborcid{0000-0003-1652-8005},
D.~Magdalinski$^{38}$\lhcborcid{0000-0001-6267-7314},
D.~Maisuzenko$^{44}$\lhcborcid{0000-0001-5704-3499},
J.J.~Malczewski$^{41}$\lhcborcid{0000-0003-2744-3656},
S.~Malde$^{64}$\lhcborcid{0000-0002-8179-0707},
L.~Malentacca$^{49}$\lhcborcid{0000-0001-6717-2980},
A.~Malinin$^{44}$\lhcborcid{0000-0002-3731-9977},
T.~Maltsev$^{44}$\lhcborcid{0000-0002-2120-5633},
G.~Manca$^{32,k}$\lhcborcid{0000-0003-1960-4413},
G.~Mancinelli$^{13}$\lhcborcid{0000-0003-1144-3678},
C.~Mancuso$^{30}$\lhcborcid{0000-0002-2490-435X},
R.~Manera~Escalero$^{46}$\lhcborcid{0000-0003-4981-6847},
F. M. ~Manganella$^{37}$\lhcborcid{0009-0003-1124-0974},
D.~Manuzzi$^{25}$\lhcborcid{0000-0002-9915-6587},
D.~Marangotto$^{30,n}$\lhcborcid{0000-0001-9099-4878},
J.F.~Marchand$^{10}$\lhcborcid{0000-0002-4111-0797},
R.~Marchevski$^{50}$\lhcborcid{0000-0003-3410-0918},
U.~Marconi$^{25}$\lhcborcid{0000-0002-5055-7224},
E.~Mariani$^{16}$\lhcborcid{0009-0002-3683-2709},
S.~Mariani$^{49}$\lhcborcid{0000-0002-7298-3101},
C.~Marin~Benito$^{46}$\lhcborcid{0000-0003-0529-6982},
J.~Marks$^{22}$\lhcborcid{0000-0002-2867-722X},
A.M.~Marshall$^{55}$\lhcborcid{0000-0002-9863-4954},
L. ~Martel$^{64}$\lhcborcid{0000-0001-8562-0038},
G.~Martelli$^{34,q}$\lhcborcid{0000-0002-6150-3168},
G.~Martellotti$^{36}$\lhcborcid{0000-0002-8663-9037},
L.~Martinazzoli$^{49}$\lhcborcid{0000-0002-8996-795X},
M.~Martinelli$^{31,o}$\lhcborcid{0000-0003-4792-9178},
D. ~Martinez~Gomez$^{79}$\lhcborcid{0009-0001-2684-9139},
D.~Martinez~Santos$^{82}$\lhcborcid{0000-0002-6438-4483},
F.~Martinez~Vidal$^{48}$\lhcborcid{0000-0001-6841-6035},
A. ~Martorell~i~Granollers$^{45}$\lhcborcid{0009-0005-6982-9006},
A.~Massafferri$^{2}$\lhcborcid{0000-0002-3264-3401},
R.~Matev$^{49}$\lhcborcid{0000-0001-8713-6119},
A.~Mathad$^{49}$\lhcborcid{0000-0002-9428-4715},
V.~Matiunin$^{44}$\lhcborcid{0000-0003-4665-5451},
C.~Matteuzzi$^{69}$\lhcborcid{0000-0002-4047-4521},
K.R.~Mattioli$^{15}$\lhcborcid{0000-0003-2222-7727},
A.~Mauri$^{62}$\lhcborcid{0000-0003-1664-8963},
E.~Maurice$^{15}$\lhcborcid{0000-0002-7366-4364},
J.~Mauricio$^{46}$\lhcborcid{0000-0002-9331-1363},
P.~Mayencourt$^{50}$\lhcborcid{0000-0002-8210-1256},
J.~Mazorra~de~Cos$^{48}$\lhcborcid{0000-0003-0525-2736},
M.~Mazurek$^{42}$\lhcborcid{0000-0002-3687-9630},
M.~McCann$^{62}$\lhcborcid{0000-0002-3038-7301},
T.H.~McGrath$^{63}$\lhcborcid{0000-0001-8993-3234},
N.T.~McHugh$^{60}$\lhcborcid{0000-0002-5477-3995},
A.~McNab$^{63}$\lhcborcid{0000-0001-5023-2086},
R.~McNulty$^{23}$\lhcborcid{0000-0001-7144-0175},
B.~Meadows$^{66}$\lhcborcid{0000-0002-1947-8034},
G.~Meier$^{19}$\lhcborcid{0000-0002-4266-1726},
D.~Melnychuk$^{42}$\lhcborcid{0000-0003-1667-7115},
F. M. ~Meng$^{4,b}$\lhcborcid{0009-0004-1533-6014},
M.~Merk$^{38,80}$\lhcborcid{0000-0003-0818-4695},
A.~Merli$^{50}$\lhcborcid{0000-0002-0374-5310},
L.~Meyer~Garcia$^{67}$\lhcborcid{0000-0002-2622-8551},
D.~Miao$^{5,7}$\lhcborcid{0000-0003-4232-5615},
H.~Miao$^{7}$\lhcborcid{0000-0002-1936-5400},
M.~Mikhasenko$^{76}$\lhcborcid{0000-0002-6969-2063},
D.A.~Milanes$^{75,x}$\lhcborcid{0000-0001-7450-1121},
A.~Minotti$^{31,o}$\lhcborcid{0000-0002-0091-5177},
E.~Minucci$^{28}$\lhcborcid{0000-0002-3972-6824},
T.~Miralles$^{11}$\lhcborcid{0000-0002-4018-1454},
B.~Mitreska$^{19}$\lhcborcid{0000-0002-1697-4999},
D.S.~Mitzel$^{19}$\lhcborcid{0000-0003-3650-2689},
A.~Modak$^{58}$\lhcborcid{0000-0003-1198-1441},
L.~Moeser$^{19}$\lhcborcid{0009-0007-2494-8241},
R.A.~Mohammed$^{64}$\lhcborcid{0000-0002-3718-4144},
R.D.~Moise$^{17}$\lhcborcid{0000-0002-5662-8804},
S.~Mokhnenko$^{44}$\lhcborcid{0000-0002-1849-1472},
E. F.~Molina~Cardenas$^{85}$\lhcborcid{0009-0002-0674-5305},
T.~Momb{\"a}cher$^{49}$\lhcborcid{0000-0002-5612-979X},
M.~Monk$^{57,1}$\lhcborcid{0000-0003-0484-0157},
S.~Monteil$^{11}$\lhcborcid{0000-0001-5015-3353},
A.~Morcillo~Gomez$^{47}$\lhcborcid{0000-0001-9165-7080},
G.~Morello$^{28}$\lhcborcid{0000-0002-6180-3697},
M.J.~Morello$^{35,r}$\lhcborcid{0000-0003-4190-1078},
M.P.~Morgenthaler$^{22}$\lhcborcid{0000-0002-7699-5724},
J.~Moron$^{40}$\lhcborcid{0000-0002-1857-1675},
W. ~Morren$^{38}$\lhcborcid{0009-0004-1863-9344},
A.B.~Morris$^{49}$\lhcborcid{0000-0002-0832-9199},
A.G.~Morris$^{13}$\lhcborcid{0000-0001-6644-9888},
R.~Mountain$^{69}$\lhcborcid{0000-0003-1908-4219},
H.~Mu$^{4,b}$\lhcborcid{0000-0001-9720-7507},
Z. M. ~Mu$^{6}$\lhcborcid{0000-0001-9291-2231},
E.~Muhammad$^{57}$\lhcborcid{0000-0001-7413-5862},
F.~Muheim$^{59}$\lhcborcid{0000-0002-1131-8909},
M.~Mulder$^{79}$\lhcborcid{0000-0001-6867-8166},
K.~M{\"u}ller$^{51}$\lhcborcid{0000-0002-5105-1305},
F.~Mu{\~n}oz-Rojas$^{9}$\lhcborcid{0000-0002-4978-602X},
R.~Murta$^{62}$\lhcborcid{0000-0002-6915-8370},
P.~Naik$^{61}$\lhcborcid{0000-0001-6977-2971},
T.~Nakada$^{50}$\lhcborcid{0009-0000-6210-6861},
R.~Nandakumar$^{58}$\lhcborcid{0000-0002-6813-6794},
T.~Nanut$^{49}$\lhcborcid{0000-0002-5728-9867},
I.~Nasteva$^{3}$\lhcborcid{0000-0001-7115-7214},
M.~Needham$^{59}$\lhcborcid{0000-0002-8297-6714},
N.~Neri$^{30,n}$\lhcborcid{0000-0002-6106-3756},
S.~Neubert$^{18}$\lhcborcid{0000-0002-0706-1944},
N.~Neufeld$^{49}$\lhcborcid{0000-0003-2298-0102},
P.~Neustroev$^{44}$,
J.~Nicolini$^{19}$\lhcborcid{0000-0001-9034-3637},
D.~Nicotra$^{80}$\lhcborcid{0000-0001-7513-3033},
E.M.~Niel$^{49}$\lhcborcid{0000-0002-6587-4695},
N.~Nikitin$^{44}$\lhcborcid{0000-0003-0215-1091},
Q.~Niu$^{73}$,
P.~Nogarolli$^{3}$\lhcborcid{0009-0001-4635-1055},
P.~Nogga$^{18}$\lhcborcid{0009-0006-2269-4666},
C.~Normand$^{55}$\lhcborcid{0000-0001-5055-7710},
J.~Novoa~Fernandez$^{47}$\lhcborcid{0000-0002-1819-1381},
G.~Nowak$^{66}$\lhcborcid{0000-0003-4864-7164},
C.~Nunez$^{85}$\lhcborcid{0000-0002-2521-9346},
H. N. ~Nur$^{60}$\lhcborcid{0000-0002-7822-523X},
A.~Oblakowska-Mucha$^{40}$\lhcborcid{0000-0003-1328-0534},
V.~Obraztsov$^{44}$\lhcborcid{0000-0002-0994-3641},
T.~Oeser$^{17}$\lhcborcid{0000-0001-7792-4082},
S.~Okamura$^{26,l}$\lhcborcid{0000-0003-1229-3093},
A.~Okhotnikov$^{44}$,
O.~Okhrimenko$^{53}$\lhcborcid{0000-0002-0657-6962},
R.~Oldeman$^{32,k}$\lhcborcid{0000-0001-6902-0710},
F.~Oliva$^{59}$\lhcborcid{0000-0001-7025-3407},
M.~Olocco$^{19}$\lhcborcid{0000-0002-6968-1217},
C.J.G.~Onderwater$^{80}$\lhcborcid{0000-0002-2310-4166},
R.H.~O'Neil$^{49}$\lhcborcid{0000-0002-9797-8464},
D.~Osthues$^{19}$\lhcborcid{0009-0004-8234-513X},
J.M.~Otalora~Goicochea$^{3}$\lhcborcid{0000-0002-9584-8500},
P.~Owen$^{51}$\lhcborcid{0000-0002-4161-9147},
A.~Oyanguren$^{48}$\lhcborcid{0000-0002-8240-7300},
O.~Ozcelik$^{59}$\lhcborcid{0000-0003-3227-9248},
F.~Paciolla$^{35,v}$\lhcborcid{0000-0002-6001-600X},
A. ~Padee$^{42}$\lhcborcid{0000-0002-5017-7168},
K.O.~Padeken$^{18}$\lhcborcid{0000-0001-7251-9125},
B.~Pagare$^{57}$\lhcborcid{0000-0003-3184-1622},
P.R.~Pais$^{22}$\lhcborcid{0009-0005-9758-742X},
T.~Pajero$^{49}$\lhcborcid{0000-0001-9630-2000},
A.~Palano$^{24}$\lhcborcid{0000-0002-6095-9593},
M.~Palutan$^{28}$\lhcborcid{0000-0001-7052-1360},
X. ~Pan$^{4,b}$\lhcborcid{0000-0002-7439-6621},
G.~Panshin$^{44}$\lhcborcid{0000-0001-9163-2051},
L.~Paolucci$^{57}$\lhcborcid{0000-0003-0465-2893},
A.~Papanestis$^{58,49}$\lhcborcid{0000-0002-5405-2901},
M.~Pappagallo$^{24,h}$\lhcborcid{0000-0001-7601-5602},
L.L.~Pappalardo$^{26,l}$\lhcborcid{0000-0002-0876-3163},
C.~Pappenheimer$^{66}$\lhcborcid{0000-0003-0738-3668},
C.~Parkes$^{63}$\lhcborcid{0000-0003-4174-1334},
D. ~Parmar$^{76}$\lhcborcid{0009-0004-8530-7630},
B.~Passalacqua$^{26,l}$\lhcborcid{0000-0003-3643-7469},
G.~Passaleva$^{27}$\lhcborcid{0000-0002-8077-8378},
D.~Passaro$^{35,r,49}$\lhcborcid{0000-0002-8601-2197},
A.~Pastore$^{24}$\lhcborcid{0000-0002-5024-3495},
M.~Patel$^{62}$\lhcborcid{0000-0003-3871-5602},
J.~Patoc$^{64}$\lhcborcid{0009-0000-1201-4918},
C.~Patrignani$^{25,j}$\lhcborcid{0000-0002-5882-1747},
A. ~Paul$^{69}$\lhcborcid{0009-0006-7202-0811},
C.J.~Pawley$^{80}$\lhcborcid{0000-0001-9112-3724},
A.~Pellegrino$^{38}$\lhcborcid{0000-0002-7884-345X},
J. ~Peng$^{5,7}$\lhcborcid{0009-0005-4236-4667},
M.~Pepe~Altarelli$^{28}$\lhcborcid{0000-0002-1642-4030},
S.~Perazzini$^{25}$\lhcborcid{0000-0002-1862-7122},
D.~Pereima$^{44}$\lhcborcid{0000-0002-7008-8082},
H. ~Pereira~Da~Costa$^{68}$\lhcborcid{0000-0002-3863-352X},
A.~Pereiro~Castro$^{47}$\lhcborcid{0000-0001-9721-3325},
P.~Perret$^{11}$\lhcborcid{0000-0002-5732-4343},
A. ~Perrevoort$^{79}$\lhcborcid{0000-0001-6343-447X},
A.~Perro$^{49,13}$\lhcborcid{0000-0002-1996-0496},
M.J.~Peters$^{66}$\lhcborcid{0009-0008-9089-1287},
K.~Petridis$^{55}$\lhcborcid{0000-0001-7871-5119},
A.~Petrolini$^{29,m}$\lhcborcid{0000-0003-0222-7594},
J. P. ~Pfaller$^{66}$\lhcborcid{0009-0009-8578-3078},
H.~Pham$^{69}$\lhcborcid{0000-0003-2995-1953},
L.~Pica$^{35,r}$\lhcborcid{0000-0001-9837-6556},
M.~Piccini$^{34}$\lhcborcid{0000-0001-8659-4409},
L. ~Piccolo$^{32}$\lhcborcid{0000-0003-1896-2892},
B.~Pietrzyk$^{10}$\lhcborcid{0000-0003-1836-7233},
G.~Pietrzyk$^{14}$\lhcborcid{0000-0001-9622-820X},
R. N.~Pilato$^{61}$\lhcborcid{0000-0002-4325-7530},
D.~Pinci$^{36}$\lhcborcid{0000-0002-7224-9708},
F.~Pisani$^{49}$\lhcborcid{0000-0002-7763-252X},
M.~Pizzichemi$^{31,o,49}$\lhcborcid{0000-0001-5189-230X},
V.~Placinta$^{43}$\lhcborcid{0000-0003-4465-2441},
M.~Plo~Casasus$^{47}$\lhcborcid{0000-0002-2289-918X},
T.~Poeschl$^{49}$\lhcborcid{0000-0003-3754-7221},
F.~Polci$^{16}$\lhcborcid{0000-0001-8058-0436},
M.~Poli~Lener$^{28}$\lhcborcid{0000-0001-7867-1232},
A.~Poluektov$^{13}$\lhcborcid{0000-0003-2222-9925},
N.~Polukhina$^{44}$\lhcborcid{0000-0001-5942-1772},
I.~Polyakov$^{44}$\lhcborcid{0000-0002-6855-7783},
E.~Polycarpo$^{3}$\lhcborcid{0000-0002-4298-5309},
S.~Ponce$^{49}$\lhcborcid{0000-0002-1476-7056},
D.~Popov$^{7}$\lhcborcid{0000-0002-8293-2922},
S.~Poslavskii$^{44}$\lhcborcid{0000-0003-3236-1452},
K.~Prasanth$^{59}$\lhcborcid{0000-0001-9923-0938},
C.~Prouve$^{82}$\lhcborcid{0000-0003-2000-6306},
D.~Provenzano$^{32,k}$\lhcborcid{0009-0005-9992-9761},
V.~Pugatch$^{53}$\lhcborcid{0000-0002-5204-9821},
G.~Punzi$^{35,s}$\lhcborcid{0000-0002-8346-9052},
S. ~Qasim$^{51}$\lhcborcid{0000-0003-4264-9724},
Q. Q. ~Qian$^{6}$\lhcborcid{0000-0001-6453-4691},
W.~Qian$^{7}$\lhcborcid{0000-0003-3932-7556},
N.~Qin$^{4,b}$\lhcborcid{0000-0001-8453-658X},
S.~Qu$^{4,b}$\lhcborcid{0000-0002-7518-0961},
R.~Quagliani$^{49}$\lhcborcid{0000-0002-3632-2453},
R.I.~Rabadan~Trejo$^{57}$\lhcborcid{0000-0002-9787-3910},
J.H.~Rademacker$^{55}$\lhcborcid{0000-0003-2599-7209},
M.~Rama$^{35}$\lhcborcid{0000-0003-3002-4719},
M. ~Ram\'{i}rez~Garc\'{i}a$^{85}$\lhcborcid{0000-0001-7956-763X},
V.~Ramos~De~Oliveira$^{70}$\lhcborcid{0000-0003-3049-7866},
M.~Ramos~Pernas$^{57}$\lhcborcid{0000-0003-1600-9432},
M.S.~Rangel$^{3}$\lhcborcid{0000-0002-8690-5198},
F.~Ratnikov$^{44}$\lhcborcid{0000-0003-0762-5583},
G.~Raven$^{39}$\lhcborcid{0000-0002-2897-5323},
M.~Rebollo~De~Miguel$^{48}$\lhcborcid{0000-0002-4522-4863},
F.~Redi$^{30,i}$\lhcborcid{0000-0001-9728-8984},
J.~Reich$^{55}$\lhcborcid{0000-0002-2657-4040},
F.~Reiss$^{20}$\lhcborcid{0000-0002-8395-7654},
Z.~Ren$^{7}$\lhcborcid{0000-0001-9974-9350},
P.K.~Resmi$^{64}$\lhcborcid{0000-0001-9025-2225},
M. ~Ribalda~Galvez$^{46}$\lhcborcid{0009-0006-0309-7639},
R.~Ribatti$^{50}$\lhcborcid{0000-0003-1778-1213},
G.~Ricart$^{15,12}$\lhcborcid{0000-0002-9292-2066},
D.~Riccardi$^{35,r}$\lhcborcid{0009-0009-8397-572X},
S.~Ricciardi$^{58}$\lhcborcid{0000-0002-4254-3658},
K.~Richardson$^{65}$\lhcborcid{0000-0002-6847-2835},
M.~Richardson-Slipper$^{59}$\lhcborcid{0000-0002-2752-001X},
K.~Rinnert$^{61}$\lhcborcid{0000-0001-9802-1122},
P.~Robbe$^{14,49}$\lhcborcid{0000-0002-0656-9033},
G.~Robertson$^{60}$\lhcborcid{0000-0002-7026-1383},
E.~Rodrigues$^{61}$\lhcborcid{0000-0003-2846-7625},
A.~Rodriguez~Alvarez$^{46}$\lhcborcid{0009-0006-1758-936X},
E.~Rodriguez~Fernandez$^{47}$\lhcborcid{0000-0002-3040-065X},
J.A.~Rodriguez~Lopez$^{75}$\lhcborcid{0000-0003-1895-9319},
E.~Rodriguez~Rodriguez$^{49}$\lhcborcid{0000-0002-7973-8061},
J.~Roensch$^{19}$\lhcborcid{0009-0001-7628-6063},
A.~Rogachev$^{44}$\lhcborcid{0000-0002-7548-6530},
A.~Rogovskiy$^{58}$\lhcborcid{0000-0002-1034-1058},
D.L.~Rolf$^{49}$\lhcborcid{0000-0001-7908-7214},
P.~Roloff$^{49}$\lhcborcid{0000-0001-7378-4350},
V.~Romanovskiy$^{66}$\lhcborcid{0000-0003-0939-4272},
A.~Romero~Vidal$^{47}$\lhcborcid{0000-0002-8830-1486},
G.~Romolini$^{26}$\lhcborcid{0000-0002-0118-4214},
F.~Ronchetti$^{50}$\lhcborcid{0000-0003-3438-9774},
T.~Rong$^{6}$\lhcborcid{0000-0002-5479-9212},
M.~Rotondo$^{28}$\lhcborcid{0000-0001-5704-6163},
S. R. ~Roy$^{22}$\lhcborcid{0000-0002-3999-6795},
M.S.~Rudolph$^{69}$\lhcborcid{0000-0002-0050-575X},
M.~Ruiz~Diaz$^{22}$\lhcborcid{0000-0001-6367-6815},
R.A.~Ruiz~Fernandez$^{47}$\lhcborcid{0000-0002-5727-4454},
J.~Ruiz~Vidal$^{83,aa}$\lhcborcid{0000-0001-8362-7164},
J.~Ryzka$^{40}$\lhcborcid{0000-0003-4235-2445},
J. J.~Saavedra-Arias$^{9}$\lhcborcid{0000-0002-2510-8929},
J.J.~Saborido~Silva$^{47}$\lhcborcid{0000-0002-6270-130X},
R.~Sadek$^{15}$\lhcborcid{0000-0003-0438-8359},
N.~Sagidova$^{44}$\lhcborcid{0000-0002-2640-3794},
D.~Sahoo$^{77}$\lhcborcid{0000-0002-5600-9413},
N.~Sahoo$^{54}$\lhcborcid{0000-0001-9539-8370},
B.~Saitta$^{32,k}$\lhcborcid{0000-0003-3491-0232},
M.~Salomoni$^{31,49,o}$\lhcborcid{0009-0007-9229-653X},
I.~Sanderswood$^{48}$\lhcborcid{0000-0001-7731-6757},
R.~Santacesaria$^{36}$\lhcborcid{0000-0003-3826-0329},
C.~Santamarina~Rios$^{47}$\lhcborcid{0000-0002-9810-1816},
M.~Santimaria$^{28}$\lhcborcid{0000-0002-8776-6759},
L.~Santoro~$^{2}$\lhcborcid{0000-0002-2146-2648},
E.~Santovetti$^{37}$\lhcborcid{0000-0002-5605-1662},
A.~Saputi$^{26,49}$\lhcborcid{0000-0001-6067-7863},
D.~Saranin$^{44}$\lhcborcid{0000-0002-9617-9986},
A.~Sarnatskiy$^{79}$\lhcborcid{0009-0007-2159-3633},
G.~Sarpis$^{59}$\lhcborcid{0000-0003-1711-2044},
M.~Sarpis$^{78}$\lhcborcid{0000-0002-6402-1674},
C.~Satriano$^{36,t}$\lhcborcid{0000-0002-4976-0460},
A.~Satta$^{37}$\lhcborcid{0000-0003-2462-913X},
M.~Saur$^{6}$\lhcborcid{0000-0001-8752-4293},
D.~Savrina$^{44}$\lhcborcid{0000-0001-8372-6031},
H.~Sazak$^{17}$\lhcborcid{0000-0003-2689-1123},
F.~Sborzacchi$^{49,28}$\lhcborcid{0009-0004-7916-2682},
L.G.~Scantlebury~Smead$^{64}$\lhcborcid{0000-0001-8702-7991},
A.~Scarabotto$^{19}$\lhcborcid{0000-0003-2290-9672},
S.~Schael$^{17}$\lhcborcid{0000-0003-4013-3468},
S.~Scherl$^{61}$\lhcborcid{0000-0003-0528-2724},
M.~Schiller$^{60}$\lhcborcid{0000-0001-8750-863X},
H.~Schindler$^{49}$\lhcborcid{0000-0002-1468-0479},
M.~Schmelling$^{21}$\lhcborcid{0000-0003-3305-0576},
B.~Schmidt$^{49}$\lhcborcid{0000-0002-8400-1566},
S.~Schmitt$^{17}$\lhcborcid{0000-0002-6394-1081},
H.~Schmitz$^{18}$,
O.~Schneider$^{50}$\lhcborcid{0000-0002-6014-7552},
A.~Schopper$^{49}$\lhcborcid{0000-0002-8581-3312},
N.~Schulte$^{19}$\lhcborcid{0000-0003-0166-2105},
S.~Schulte$^{50}$\lhcborcid{0009-0001-8533-0783},
M.H.~Schune$^{14}$\lhcborcid{0000-0002-3648-0830},
R.~Schwemmer$^{49}$\lhcborcid{0009-0005-5265-9792},
G.~Schwering$^{17}$\lhcborcid{0000-0003-1731-7939},
B.~Sciascia$^{28}$\lhcborcid{0000-0003-0670-006X},
A.~Sciuccati$^{49}$\lhcborcid{0000-0002-8568-1487},
I.~Segal$^{76}$\lhcborcid{0000-0001-8605-3020},
S.~Sellam$^{47}$\lhcborcid{0000-0003-0383-1451},
A.~Semennikov$^{44}$\lhcborcid{0000-0003-1130-2197},
T.~Senger$^{51}$\lhcborcid{0009-0006-2212-6431},
M.~Senghi~Soares$^{39}$\lhcborcid{0000-0001-9676-6059},
A.~Sergi$^{29,m}$\lhcborcid{0000-0001-9495-6115},
N.~Serra$^{51}$\lhcborcid{0000-0002-5033-0580},
L.~Sestini$^{27}$\lhcborcid{0000-0002-1127-5144},
A.~Seuthe$^{19}$\lhcborcid{0000-0002-0736-3061},
Y.~Shang$^{6}$\lhcborcid{0000-0001-7987-7558},
D.M.~Shangase$^{85}$\lhcborcid{0000-0002-0287-6124},
M.~Shapkin$^{44}$\lhcborcid{0000-0002-4098-9592},
R. S. ~Sharma$^{69}$\lhcborcid{0000-0003-1331-1791},
I.~Shchemerov$^{44}$\lhcborcid{0000-0001-9193-8106},
L.~Shchutska$^{50}$\lhcborcid{0000-0003-0700-5448},
T.~Shears$^{61}$\lhcborcid{0000-0002-2653-1366},
L.~Shekhtman$^{44}$\lhcborcid{0000-0003-1512-9715},
Z.~Shen$^{6}$\lhcborcid{0000-0003-1391-5384},
S.~Sheng$^{5,7}$\lhcborcid{0000-0002-1050-5649},
V.~Shevchenko$^{44}$\lhcborcid{0000-0003-3171-9125},
B.~Shi$^{7}$\lhcborcid{0000-0002-5781-8933},
Q.~Shi$^{7}$\lhcborcid{0000-0001-7915-8211},
Y.~Shimizu$^{14}$\lhcborcid{0000-0002-4936-1152},
E.~Shmanin$^{25}$\lhcborcid{0000-0002-8868-1730},
R.~Shorkin$^{44}$\lhcborcid{0000-0001-8881-3943},
J.D.~Shupperd$^{69}$\lhcborcid{0009-0006-8218-2566},
R.~Silva~Coutinho$^{69}$\lhcborcid{0000-0002-1545-959X},
G.~Simi$^{33,p}$\lhcborcid{0000-0001-6741-6199},
S.~Simone$^{24,h}$\lhcborcid{0000-0003-3631-8398},
N.~Skidmore$^{57}$\lhcborcid{0000-0003-3410-0731},
T.~Skwarnicki$^{69}$\lhcborcid{0000-0002-9897-9506},
M.W.~Slater$^{54}$\lhcborcid{0000-0002-2687-1950},
J.C.~Smallwood$^{64}$\lhcborcid{0000-0003-2460-3327},
E.~Smith$^{65}$\lhcborcid{0000-0002-9740-0574},
K.~Smith$^{68}$\lhcborcid{0000-0002-1305-3377},
M.~Smith$^{62}$\lhcborcid{0000-0002-3872-1917},
A.~Snoch$^{38}$\lhcborcid{0000-0001-6431-6360},
L.~Soares~Lavra$^{59}$\lhcborcid{0000-0002-2652-123X},
M.D.~Sokoloff$^{66}$\lhcborcid{0000-0001-6181-4583},
F.J.P.~Soler$^{60}$\lhcborcid{0000-0002-4893-3729},
A.~Solomin$^{44,55}$\lhcborcid{0000-0003-0644-3227},
A.~Solovev$^{44}$\lhcborcid{0000-0002-5355-5996},
I.~Solovyev$^{44}$\lhcborcid{0000-0003-4254-6012},
N. S. ~Sommerfeld$^{18}$\lhcborcid{0009-0006-7822-2860},
R.~Song$^{1}$\lhcborcid{0000-0002-8854-8905},
Y.~Song$^{50}$\lhcborcid{0000-0003-0256-4320},
Y.~Song$^{4,b}$\lhcborcid{0000-0003-1959-5676},
Y. S. ~Song$^{6}$\lhcborcid{0000-0003-3471-1751},
F.L.~Souza~De~Almeida$^{69}$\lhcborcid{0000-0001-7181-6785},
B.~Souza~De~Paula$^{3}$\lhcborcid{0009-0003-3794-3408},
E.~Spadaro~Norella$^{29,m}$\lhcborcid{0000-0002-1111-5597},
E.~Spedicato$^{25}$\lhcborcid{0000-0002-4950-6665},
J.G.~Speer$^{19}$\lhcborcid{0000-0002-6117-7307},
E.~Spiridenkov$^{44}$,
P.~Spradlin$^{60}$\lhcborcid{0000-0002-5280-9464},
V.~Sriskaran$^{49}$\lhcborcid{0000-0002-9867-0453},
F.~Stagni$^{49}$\lhcborcid{0000-0002-7576-4019},
M.~Stahl$^{76}$\lhcborcid{0000-0001-8476-8188},
S.~Stahl$^{49}$\lhcborcid{0000-0002-8243-400X},
S.~Stanislaus$^{64}$\lhcborcid{0000-0003-1776-0498},
M. ~Stefaniak$^{86}$\lhcborcid{0000-0002-5820-1054},
E.N.~Stein$^{49}$\lhcborcid{0000-0001-5214-8865},
O.~Steinkamp$^{51}$\lhcborcid{0000-0001-7055-6467},
O.~Stenyakin$^{44}$,
H.~Stevens$^{19}$\lhcborcid{0000-0002-9474-9332},
D.~Strekalina$^{44}$\lhcborcid{0000-0003-3830-4889},
Y.~Su$^{7}$\lhcborcid{0000-0002-2739-7453},
F.~Suljik$^{64}$\lhcborcid{0000-0001-6767-7698},
J.~Sun$^{32}$\lhcborcid{0000-0002-6020-2304},
L.~Sun$^{74}$\lhcborcid{0000-0002-0034-2567},
D.~Sundfeld$^{2}$\lhcborcid{0000-0002-5147-3698},
W.~Sutcliffe$^{51}$\lhcborcid{0000-0002-9795-3582},
K.~Swientek$^{40}$\lhcborcid{0000-0001-6086-4116},
F.~Swystun$^{56}$\lhcborcid{0009-0006-0672-7771},
A.~Szabelski$^{42}$\lhcborcid{0000-0002-6604-2938},
T.~Szumlak$^{40}$\lhcborcid{0000-0002-2562-7163},
Y.~Tan$^{4,b}$\lhcborcid{0000-0003-3860-6545},
Y.~Tang$^{74}$\lhcborcid{0000-0002-6558-6730},
M.D.~Tat$^{22}$\lhcborcid{0000-0002-6866-7085},
A.~Terentev$^{44}$\lhcborcid{0000-0003-2574-8560},
F.~Terzuoli$^{35,v,49}$\lhcborcid{0000-0002-9717-225X},
F.~Teubert$^{49}$\lhcborcid{0000-0003-3277-5268},
E.~Thomas$^{49}$\lhcborcid{0000-0003-0984-7593},
D.J.D.~Thompson$^{54}$\lhcborcid{0000-0003-1196-5943},
H.~Tilquin$^{62}$\lhcborcid{0000-0003-4735-2014},
V.~Tisserand$^{11}$\lhcborcid{0000-0003-4916-0446},
S.~T'Jampens$^{10}$\lhcborcid{0000-0003-4249-6641},
M.~Tobin$^{5,49}$\lhcborcid{0000-0002-2047-7020},
L.~Tomassetti$^{26,l}$\lhcborcid{0000-0003-4184-1335},
G.~Tonani$^{30,n}$\lhcborcid{0000-0001-7477-1148},
X.~Tong$^{6}$\lhcborcid{0000-0002-5278-1203},
T.~Tork$^{30}$\lhcborcid{0000-0001-9753-329X},
D.~Torres~Machado$^{2}$\lhcborcid{0000-0001-7030-6468},
L.~Toscano$^{19}$\lhcborcid{0009-0007-5613-6520},
D.Y.~Tou$^{4,b}$\lhcborcid{0000-0002-4732-2408},
C.~Trippl$^{45}$\lhcborcid{0000-0003-3664-1240},
G.~Tuci$^{22}$\lhcborcid{0000-0002-0364-5758},
N.~Tuning$^{38}$\lhcborcid{0000-0003-2611-7840},
L.H.~Uecker$^{22}$\lhcborcid{0000-0003-3255-9514},
A.~Ukleja$^{40}$\lhcborcid{0000-0003-0480-4850},
D.J.~Unverzagt$^{22}$\lhcborcid{0000-0002-1484-2546},
B. ~Urbach$^{59}$\lhcborcid{0009-0001-4404-561X},
A.~Usachov$^{39}$\lhcborcid{0000-0002-5829-6284},
A.~Ustyuzhanin$^{44}$\lhcborcid{0000-0001-7865-2357},
U.~Uwer$^{22}$\lhcborcid{0000-0002-8514-3777},
V.~Vagnoni$^{25}$\lhcborcid{0000-0003-2206-311X},
V. ~Valcarce~Cadenas$^{47}$\lhcborcid{0009-0006-3241-8964},
G.~Valenti$^{25}$\lhcborcid{0000-0002-6119-7535},
N.~Valls~Canudas$^{49}$\lhcborcid{0000-0001-8748-8448},
J.~van~Eldik$^{49}$\lhcborcid{0000-0002-3221-7664},
H.~Van~Hecke$^{68}$\lhcborcid{0000-0001-7961-7190},
E.~van~Herwijnen$^{62}$\lhcborcid{0000-0001-8807-8811},
C.B.~Van~Hulse$^{47,y}$\lhcborcid{0000-0002-5397-6782},
R.~Van~Laak$^{50}$\lhcborcid{0000-0002-7738-6066},
M.~van~Veghel$^{38}$\lhcborcid{0000-0001-6178-6623},
G.~Vasquez$^{51}$\lhcborcid{0000-0002-3285-7004},
R.~Vazquez~Gomez$^{46}$\lhcborcid{0000-0001-5319-1128},
P.~Vazquez~Regueiro$^{47}$\lhcborcid{0000-0002-0767-9736},
C.~V{\'a}zquez~Sierra$^{47}$\lhcborcid{0000-0002-5865-0677},
S.~Vecchi$^{26}$\lhcborcid{0000-0002-4311-3166},
J.J.~Velthuis$^{55}$\lhcborcid{0000-0002-4649-3221},
M.~Veltri$^{27,w}$\lhcborcid{0000-0001-7917-9661},
A.~Venkateswaran$^{50}$\lhcborcid{0000-0001-6950-1477},
M.~Verdoglia$^{32}$\lhcborcid{0009-0006-3864-8365},
M.~Vesterinen$^{57}$\lhcborcid{0000-0001-7717-2765},
D. ~Vico~Benet$^{64}$\lhcborcid{0009-0009-3494-2825},
P. ~Vidrier~Villalba$^{46}$\lhcborcid{0009-0005-5503-8334},
M.~Vieites~Diaz$^{47}$\lhcborcid{0000-0002-0944-4340},
X.~Vilasis-Cardona$^{45}$\lhcborcid{0000-0002-1915-9543},
E.~Vilella~Figueras$^{61}$\lhcborcid{0000-0002-7865-2856},
A.~Villa$^{25}$\lhcborcid{0000-0002-9392-6157},
P.~Vincent$^{16}$\lhcborcid{0000-0002-9283-4541},
F.C.~Volle$^{54}$\lhcborcid{0000-0003-1828-3881},
D.~vom~Bruch$^{13}$\lhcborcid{0000-0001-9905-8031},
N.~Voropaev$^{44}$\lhcborcid{0000-0002-2100-0726},
K.~Vos$^{80}$\lhcborcid{0000-0002-4258-4062},
C.~Vrahas$^{59}$\lhcborcid{0000-0001-6104-1496},
J.~Wagner$^{19}$\lhcborcid{0000-0002-9783-5957},
J.~Walsh$^{35}$\lhcborcid{0000-0002-7235-6976},
E.J.~Walton$^{1,57}$\lhcborcid{0000-0001-6759-2504},
G.~Wan$^{6}$\lhcborcid{0000-0003-0133-1664},
C.~Wang$^{22}$\lhcborcid{0000-0002-5909-1379},
G.~Wang$^{8}$\lhcborcid{0000-0001-6041-115X},
H.~Wang$^{73}$\lhcborcid{0009-0008-3130-0600},
J.~Wang$^{6}$\lhcborcid{0000-0001-7542-3073},
J.~Wang$^{5}$\lhcborcid{0000-0002-6391-2205},
J.~Wang$^{4,b}$\lhcborcid{0000-0002-3281-8136},
J.~Wang$^{74}$\lhcborcid{0000-0001-6711-4465},
M.~Wang$^{49}$\lhcborcid{0000-0003-4062-710X},
N. W. ~Wang$^{7}$\lhcborcid{0000-0002-6915-6607},
R.~Wang$^{55}$\lhcborcid{0000-0002-2629-4735},
X.~Wang$^{8}$\lhcborcid{0009-0006-3560-1596},
X.~Wang$^{72}$\lhcborcid{0000-0002-2399-7646},
X. W. ~Wang$^{62}$\lhcborcid{0000-0001-9565-8312},
Y.~Wang$^{6}$\lhcborcid{0009-0003-2254-7162},
Y. W. ~Wang$^{73}$,
Z.~Wang$^{14}$\lhcborcid{0000-0002-5041-7651},
Z.~Wang$^{4,b}$\lhcborcid{0000-0003-0597-4878},
Z.~Wang$^{30}$\lhcborcid{0000-0003-4410-6889},
J.A.~Ward$^{57,1}$\lhcborcid{0000-0003-4160-9333},
M.~Waterlaat$^{49}$\lhcborcid{0000-0002-2778-0102},
N.K.~Watson$^{54}$\lhcborcid{0000-0002-8142-4678},
D.~Websdale$^{62}$\lhcborcid{0000-0002-4113-1539},
Y.~Wei$^{6}$\lhcborcid{0000-0001-6116-3944},
J.~Wendel$^{82}$\lhcborcid{0000-0003-0652-721X},
B.D.C.~Westhenry$^{55}$\lhcborcid{0000-0002-4589-2626},
C.~White$^{56}$\lhcborcid{0009-0002-6794-9547},
M.~Whitehead$^{60}$\lhcborcid{0000-0002-2142-3673},
E.~Whiter$^{54}$\lhcborcid{0009-0003-3902-8123},
A.R.~Wiederhold$^{63}$\lhcborcid{0000-0002-1023-1086},
D.~Wiedner$^{19}$\lhcborcid{0000-0002-4149-4137},
G.~Wilkinson$^{64}$\lhcborcid{0000-0001-5255-0619},
M.K.~Wilkinson$^{66}$\lhcborcid{0000-0001-6561-2145},
M.~Williams$^{65}$\lhcborcid{0000-0001-8285-3346},
M. J.~Williams$^{49}$\lhcborcid{0000-0001-7765-8941},
M.R.J.~Williams$^{59}$\lhcborcid{0000-0001-5448-4213},
R.~Williams$^{56}$\lhcborcid{0000-0002-2675-3567},
Z. ~Williams$^{55}$\lhcborcid{0009-0009-9224-4160},
F.F.~Wilson$^{58}$\lhcborcid{0000-0002-5552-0842},
M.~Winn$^{12}$\lhcborcid{0000-0002-2207-0101},
W.~Wislicki$^{42}$\lhcborcid{0000-0001-5765-6308},
M.~Witek$^{41}$\lhcborcid{0000-0002-8317-385X},
L.~Witola$^{22}$\lhcborcid{0000-0001-9178-9921},
G.~Wormser$^{14}$\lhcborcid{0000-0003-4077-6295},
S.A.~Wotton$^{56}$\lhcborcid{0000-0003-4543-8121},
H.~Wu$^{69}$\lhcborcid{0000-0002-9337-3476},
J.~Wu$^{8}$\lhcborcid{0000-0002-4282-0977},
X.~Wu$^{74}$\lhcborcid{0000-0002-0654-7504},
Y.~Wu$^{6}$\lhcborcid{0000-0003-3192-0486},
Z.~Wu$^{7}$\lhcborcid{0000-0001-6756-9021},
K.~Wyllie$^{49}$\lhcborcid{0000-0002-2699-2189},
S.~Xian$^{72}$\lhcborcid{0009-0009-9115-1122},
Z.~Xiang$^{5}$\lhcborcid{0000-0002-9700-3448},
Y.~Xie$^{8}$\lhcborcid{0000-0001-5012-4069},
T. X. ~Xing$^{30}$\lhcborcid{0009-0006-7038-0143},
A.~Xu$^{35}$\lhcborcid{0000-0002-8521-1688},
L.~Xu$^{4,b}$\lhcborcid{0000-0003-2800-1438},
L.~Xu$^{4,b}$\lhcborcid{0000-0002-0241-5184},
M.~Xu$^{57}$\lhcborcid{0000-0001-8885-565X},
Z.~Xu$^{49}$\lhcborcid{0000-0002-7531-6873},
Z.~Xu$^{7}$\lhcborcid{0000-0001-9558-1079},
Z.~Xu$^{5}$\lhcborcid{0000-0001-9602-4901},
K. ~Yang$^{62}$\lhcborcid{0000-0001-5146-7311},
S.~Yang$^{7}$\lhcborcid{0000-0003-2505-0365},
X.~Yang$^{6}$\lhcborcid{0000-0002-7481-3149},
Y.~Yang$^{29,m}$\lhcborcid{0000-0002-8917-2620},
Z.~Yang$^{6}$\lhcborcid{0000-0003-2937-9782},
V.~Yeroshenko$^{14}$\lhcborcid{0000-0002-8771-0579},
H.~Yeung$^{63}$\lhcborcid{0000-0001-9869-5290},
H.~Yin$^{8}$\lhcborcid{0000-0001-6977-8257},
X. ~Yin$^{7}$\lhcborcid{0009-0003-1647-2942},
C. Y. ~Yu$^{6}$\lhcborcid{0000-0002-4393-2567},
J.~Yu$^{71}$\lhcborcid{0000-0003-1230-3300},
X.~Yuan$^{5}$\lhcborcid{0000-0003-0468-3083},
Y~Yuan$^{5,7}$\lhcborcid{0009-0000-6595-7266},
E.~Zaffaroni$^{50}$\lhcborcid{0000-0003-1714-9218},
M.~Zavertyaev$^{21}$\lhcborcid{0000-0002-4655-715X},
M.~Zdybal$^{41}$\lhcborcid{0000-0002-1701-9619},
F.~Zenesini$^{25}$\lhcborcid{0009-0001-2039-9739},
C. ~Zeng$^{5,7}$\lhcborcid{0009-0007-8273-2692},
M.~Zeng$^{4,b}$\lhcborcid{0000-0001-9717-1751},
C.~Zhang$^{6}$\lhcborcid{0000-0002-9865-8964},
D.~Zhang$^{8}$\lhcborcid{0000-0002-8826-9113},
J.~Zhang$^{7}$\lhcborcid{0000-0001-6010-8556},
L.~Zhang$^{4,b}$\lhcborcid{0000-0003-2279-8837},
S.~Zhang$^{71}$\lhcborcid{0000-0002-9794-4088},
S.~Zhang$^{64}$\lhcborcid{0000-0002-2385-0767},
Y.~Zhang$^{6}$\lhcborcid{0000-0002-0157-188X},
Y. Z. ~Zhang$^{4,b}$\lhcborcid{0000-0001-6346-8872},
Z.~Zhang$^{4,b}$\lhcborcid{0000-0002-1630-0986},
Y.~Zhao$^{22}$\lhcborcid{0000-0002-8185-3771},
A.~Zhelezov$^{22}$\lhcborcid{0000-0002-2344-9412},
S. Z. ~Zheng$^{6}$\lhcborcid{0009-0001-4723-095X},
X. Z. ~Zheng$^{4,b}$\lhcborcid{0000-0001-7647-7110},
Y.~Zheng$^{7}$\lhcborcid{0000-0003-0322-9858},
T.~Zhou$^{6}$\lhcborcid{0000-0002-3804-9948},
X.~Zhou$^{8}$\lhcborcid{0009-0005-9485-9477},
Y.~Zhou$^{7}$\lhcborcid{0000-0003-2035-3391},
V.~Zhovkovska$^{57}$\lhcborcid{0000-0002-9812-4508},
L. Z. ~Zhu$^{7}$\lhcborcid{0000-0003-0609-6456},
X.~Zhu$^{4,b}$\lhcborcid{0000-0002-9573-4570},
X.~Zhu$^{8}$\lhcborcid{0000-0002-4485-1478},
V.~Zhukov$^{17}$\lhcborcid{0000-0003-0159-291X},
J.~Zhuo$^{48}$\lhcborcid{0000-0002-6227-3368},
Q.~Zou$^{5,7}$\lhcborcid{0000-0003-0038-5038},
D.~Zuliani$^{33,p}$\lhcborcid{0000-0002-1478-4593},
G.~Zunica$^{50}$\lhcborcid{0000-0002-5972-6290}.\bigskip

{\footnotesize \it

$^{1}$School of Physics and Astronomy, Monash University, Melbourne, Australia\\
$^{2}$Centro Brasileiro de Pesquisas F{\'\i}sicas (CBPF), Rio de Janeiro, Brazil\\
$^{3}$Universidade Federal do Rio de Janeiro (UFRJ), Rio de Janeiro, Brazil\\
$^{4}$Department of Engineering Physics, Tsinghua University, Beijing, China\\
$^{5}$Institute Of High Energy Physics (IHEP), Beijing, China\\
$^{6}$School of Physics State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing, China\\
$^{7}$University of Chinese Academy of Sciences, Beijing, China\\
$^{8}$Institute of Particle Physics, Central China Normal University, Wuhan, Hubei, China\\
$^{9}$Consejo Nacional de Rectores  (CONARE), San Jose, Costa Rica\\
$^{10}$Universit{\'e} Savoie Mont Blanc, CNRS, IN2P3-LAPP, Annecy, France\\
$^{11}$Universit{\'e} Clermont Auvergne, CNRS/IN2P3, LPC, Clermont-Ferrand, France\\
$^{12}$Université Paris-Saclay, Centre d'Etudes de Saclay (CEA), IRFU, Saclay, France, Gif-Sur-Yvette, France\\
$^{13}$Aix Marseille Univ, CNRS/IN2P3, CPPM, Marseille, France\\
$^{14}$Universit{\'e} Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France\\
$^{15}$Laboratoire Leprince-Ringuet, CNRS/IN2P3, Ecole Polytechnique, Institut Polytechnique de Paris, Palaiseau, France\\
$^{16}$LPNHE, Sorbonne Universit{\'e}, Paris Diderot Sorbonne Paris Cit{\'e}, CNRS/IN2P3, Paris, France\\
$^{17}$I. Physikalisches Institut, RWTH Aachen University, Aachen, Germany\\
$^{18}$Universit{\"a}t Bonn - Helmholtz-Institut f{\"u}r Strahlen und Kernphysik, Bonn, Germany\\
$^{19}$Fakult{\"a}t Physik, Technische Universit{\"a}t Dortmund, Dortmund, Germany\\
$^{20}$Physikalisches Institut, Albert-Ludwigs-Universit{\"a}t Freiburg, Freiburg, Germany\\
$^{21}$Max-Planck-Institut f{\"u}r Kernphysik (MPIK), Heidelberg, Germany\\
$^{22}$Physikalisches Institut, Ruprecht-Karls-Universit{\"a}t Heidelberg, Heidelberg, Germany\\
$^{23}$School of Physics, University College Dublin, Dublin, Ireland\\
$^{24}$INFN Sezione di Bari, Bari, Italy\\
$^{25}$INFN Sezione di Bologna, Bologna, Italy\\
$^{26}$INFN Sezione di Ferrara, Ferrara, Italy\\
$^{27}$INFN Sezione di Firenze, Firenze, Italy\\
$^{28}$INFN Laboratori Nazionali di Frascati, Frascati, Italy\\
$^{29}$INFN Sezione di Genova, Genova, Italy\\
$^{30}$INFN Sezione di Milano, Milano, Italy\\
$^{31}$INFN Sezione di Milano-Bicocca, Milano, Italy\\
$^{32}$INFN Sezione di Cagliari, Monserrato, Italy\\
$^{33}$INFN Sezione di Padova, Padova, Italy\\
$^{34}$INFN Sezione di Perugia, Perugia, Italy\\
$^{35}$INFN Sezione di Pisa, Pisa, Italy\\
$^{36}$INFN Sezione di Roma La Sapienza, Roma, Italy\\
$^{37}$INFN Sezione di Roma Tor Vergata, Roma, Italy\\
$^{38}$Nikhef National Institute for Subatomic Physics, Amsterdam, Netherlands\\
$^{39}$Nikhef National Institute for Subatomic Physics and VU University Amsterdam, Amsterdam, Netherlands\\
$^{40}$AGH - University of Krakow, Faculty of Physics and Applied Computer Science, Krak{\'o}w, Poland\\
$^{41}$Henryk Niewodniczanski Institute of Nuclear Physics  Polish Academy of Sciences, Krak{\'o}w, Poland\\
$^{42}$National Center for Nuclear Research (NCBJ), Warsaw, Poland\\
$^{43}$Horia Hulubei National Institute of Physics and Nuclear Engineering, Bucharest-Magurele, Romania\\
$^{44}$Authors affiliated with an institute formerly covered by a cooperation agreement with CERN.\\
$^{45}$DS4DS, La Salle, Universitat Ramon Llull, Barcelona, Spain\\
$^{46}$ICCUB, Universitat de Barcelona, Barcelona, Spain\\
$^{47}$Instituto Galego de F{\'\i}sica de Altas Enerx{\'\i}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain\\
$^{48}$Instituto de Fisica Corpuscular, Centro Mixto Universidad de Valencia - CSIC, Valencia, Spain\\
$^{49}$European Organization for Nuclear Research (CERN), Geneva, Switzerland\\
$^{50}$Institute of Physics, Ecole Polytechnique  F{\'e}d{\'e}rale de Lausanne (EPFL), Lausanne, Switzerland\\
$^{51}$Physik-Institut, Universit{\"a}t Z{\"u}rich, Z{\"u}rich, Switzerland\\
$^{52}$NSC Kharkiv Institute of Physics and Technology (NSC KIPT), Kharkiv, Ukraine\\
$^{53}$Institute for Nuclear Research of the National Academy of Sciences (KINR), Kyiv, Ukraine\\
$^{54}$School of Physics and Astronomy, University of Birmingham, Birmingham, United Kingdom\\
$^{55}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom\\
$^{56}$Cavendish Laboratory, University of Cambridge, Cambridge, United Kingdom\\
$^{57}$Department of Physics, University of Warwick, Coventry, United Kingdom\\
$^{58}$STFC Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$^{59}$School of Physics and Astronomy, University of Edinburgh, Edinburgh, United Kingdom\\
$^{60}$School of Physics and Astronomy, University of Glasgow, Glasgow, United Kingdom\\
$^{61}$Oliver Lodge Laboratory, University of Liverpool, Liverpool, United Kingdom\\
$^{62}$Imperial College London, London, United Kingdom\\
$^{63}$Department of Physics and Astronomy, University of Manchester, Manchester, United Kingdom\\
$^{64}$Department of Physics, University of Oxford, Oxford, United Kingdom\\
$^{65}$Massachusetts Institute of Technology, Cambridge, MA, United States\\
$^{66}$University of Cincinnati, Cincinnati, OH, United States\\
$^{67}$University of Maryland, College Park, MD, United States\\
$^{68}$Los Alamos National Laboratory (LANL), Los Alamos, NM, United States\\
$^{69}$Syracuse University, Syracuse, NY, United States\\
$^{70}$Pontif{\'\i}cia Universidade Cat{\'o}lica do Rio de Janeiro (PUC-Rio), Rio de Janeiro, Brazil, associated to $^{3}$\\
$^{71}$School of Physics and Electronics, Hunan University, Changsha City, China, associated to $^{8}$\\
$^{72}$Guangdong Provincial Key Laboratory of Nuclear Science, Guangdong-Hong Kong Joint Laboratory of Quantum Matter, Institute of Quantum Matter, South China Normal University, Guangzhou, China, associated to $^{4}$\\
$^{73}$Lanzhou University, Lanzhou, China, associated to $^{5}$\\
$^{74}$School of Physics and Technology, Wuhan University, Wuhan, China, associated to $^{4}$\\
$^{75}$Departamento de Fisica , Universidad Nacional de Colombia, Bogota, Colombia, associated to $^{16}$\\
$^{76}$Ruhr Universitaet Bochum, Fakultaet f. Physik und Astronomie, Bochum, Germany, associated to $^{19}$\\
$^{77}$Eotvos Lorand University, Budapest, Hungary, associated to $^{49}$\\
$^{78}$Vilnius University, Vilnius, Lithuania, associated to $^{20}$\\
$^{79}$Van Swinderen Institute, University of Groningen, Groningen, Netherlands, associated to $^{38}$\\
$^{80}$Universiteit Maastricht, Maastricht, Netherlands, associated to $^{38}$\\
$^{81}$Tadeusz Kosciuszko Cracow University of Technology, Cracow, Poland, associated to $^{41}$\\
$^{82}$Universidade da Coru{\~n}a, A Coru{\~n}a, Spain, associated to $^{45}$\\
$^{83}$Department of Physics and Astronomy, Uppsala University, Uppsala, Sweden, associated to $^{60}$\\
$^{84}$Taras Schevchenko University of Kyiv, Faculty of Physics, Kyiv, Ukraine, associated to $^{14}$\\
$^{85}$University of Michigan, Ann Arbor, MI, United States, associated to $^{69}$\\
$^{86}$Ohio State University, Columbus, United States, associated to $^{68}$\\
\bigskip
$^{a}$Centro Federal de Educac{\~a}o Tecnol{\'o}gica Celso Suckow da Fonseca, Rio De Janeiro, Brazil\\
$^{b}$Center for High Energy Physics, Tsinghua University, Beijing, China\\
$^{c}$Hangzhou Institute for Advanced Study, UCAS, Hangzhou, China\\
$^{d}$School of Physics and Electronics, Henan University , Kaifeng, China\\
$^{e}$LIP6, Sorbonne Universit{\'e}, Paris, France\\
$^{f}$Lamarr Institute for Machine Learning and Artificial Intelligence, Dortmund, Germany\\
$^{g}$Universidad Nacional Aut{\'o}noma de Honduras, Tegucigalpa, Honduras\\
$^{h}$Universit{\`a} di Bari, Bari, Italy\\
$^{i}$Universit\`{a} di Bergamo, Bergamo, Italy\\
$^{j}$Universit{\`a} di Bologna, Bologna, Italy\\
$^{k}$Universit{\`a} di Cagliari, Cagliari, Italy\\
$^{l}$Universit{\`a} di Ferrara, Ferrara, Italy\\
$^{m}$Universit{\`a} di Genova, Genova, Italy\\
$^{n}$Universit{\`a} degli Studi di Milano, Milano, Italy\\
$^{o}$Universit{\`a} degli Studi di Milano-Bicocca, Milano, Italy\\
$^{p}$Universit{\`a} di Padova, Padova, Italy\\
$^{q}$Universit{\`a}  di Perugia, Perugia, Italy\\
$^{r}$Scuola Normale Superiore, Pisa, Italy\\
$^{s}$Universit{\`a} di Pisa, Pisa, Italy\\
$^{t}$Universit{\`a} della Basilicata, Potenza, Italy\\
$^{u}$Universit{\`a} di Roma Tor Vergata, Roma, Italy\\
$^{v}$Universit{\`a} di Siena, Siena, Italy\\
$^{w}$Universit{\`a} di Urbino, Urbino, Italy\\
$^{x}$Universidad de Ingenier\'{i}a y Tecnolog\'{i}a (UTEC), Lima, Peru\\
$^{y}$Universidad de Alcal{\'a}, Alcal{\'a} de Henares , Spain\\
$^{z}$Facultad de Ciencias Fisicas, Madrid, Spain\\
$^{aa}$Department of Physics/Division of Particle Physics, Lund, Sweden\\
\medskip
$ ^{\dagger}$Deceased
}
\end{flushleft}

==> Authorship_LHCb-PAPER-20YY-nnn.tex <==
% ===============================================================================
% Purpose: example of authorlist for LHCb template
% Author:
% Created on: 2009-09-24
% ===============================================================================

%\documentclass[a4paper]{article}
%\setlength{\oddsidemargin}{0cm}
%\setlength{\evensidemargin}{0cm}
%\setlength{\textwidth}{16.5cm}
%\setlength{\parindent}{0cm}
%\begin{document}
\centerline{\large\normalfont\bfseries LHCb collaboration}
\begin{flushleft}
\small
%-- LHCb Authorlist, Example typesetting
%-- 
A.~N.~Other$^{1}$.\bigskip\newline{\it
\footnotesize
$ ^{1}$University of nowhere\\
}
%-- 
%-- 
\end{flushleft}
%\end{document}



